Characteristic Gluing with $\Lambda$ 1. Linearised Einstein equations on four-dimensional spacetimes

We establish a gluing theorem for linearised vacuum gravitational fields in Bondi gauge on a class of characteristic surfaces in static vacuum four-dimensional backgrounds with cosmological constant $\Lambda \in \mathbb{R}$ and arbitrary topology of the compact cross-sections of the null hypersurface. This generalises and complements, in the linearised case, the pioneering analysis of Aretakis, Czimek and Rodnianski, carried-out on light-cones in Minkowski spacetime.

==> 4DDetailsOfRecursion.tex <==

\reject







Working out the recursion coefficients:



\begin{align}
    \overadd{i+1}{\psi}(s,r)&=
    \green{\sum_{k=0}^{i}\overadd{i,k,0}{\psi}(r)\partial^k_r\big(\overadd{1,0}{\psi}(s,r)\big)}
    +\overadd{i}{\psi}(s,r)\overadd{1,0,0}{\psi}(s)
   \nonumber
\\
    &\quad
    - \partial_s\bigg(\overadd{i}{\psi}(s,r)\overadd{1,1,0}{\psi}(s)\bigg)
    +\int_s^r\overadd{i}{\psi}(y,r)\overadd{1}{\psi}(s,y)\,dy
\end{align}
%

%
\begin{align}
    \overadd{i+1,1}{\psi}_p(s,r)
    &= \green{\sum_{k=0}^{i-1}\overadd{i,k,1}{\psi}(r)\partial^k_r\big(\overadd{1,0}{\psi}(s,r)\big)}
    +\green{\sum_{\ell=0}^{i}\overset{(i,\ell,0)}{\psi}(r) \partial_r^{\ell}\big(\overadd{1,1}{\psi}_p(s,r)\big)}
    \nonumber
\\
    &\quad
    +\overadd{i,1}{\psi}_p(s,r)\overadd{1,0,0}{\psi}(s)
    -\partial_s\bigg(\overadd{i,1}{\psi}_p(s,r)\overadd{1,1,0}{\psi}(s)\bigg)
    \nonumber
\\
    &+\int_s^r\overadd{i}{\psi}(y,r)\overadd{1,1}{\psi}_p(s,y)\,dy
    +\int_s^r\overadd{i,1}{\psi}_p(y,r)\overadd{1}{\psi}(s,y)\,dy
    \,,
\\
    \overadd{i+1,j}{\psi}_p(s,r)
    &=\green{\sum_{k=0}^{i-j}\overadd{i,k,j}{\psi}(r)\partial^k_r\big(\overadd{1,0}{\psi}(s,r)\big)}
    +\green{\sum_{\ell=0}^{i-j+1}\overset{(i,\ell,j-1)}{\psi}(r) \partial_r^{\ell}\big(\overadd{1,1}{\psi}_p(s,r)\big)}
    \nonumber
\\
    &\quad 
    +\overadd{i,j}{\psi}_p(s,r)\overadd{1,0,0}{\psi}(s)
    -\partial_s\bigg(\overadd{i,j}{\psi}_p(s,r)\overadd{1,1,0}{\psi}(s)\bigg)
    \nonumber
\\
    &
    +\int_s^r\overadd{i,j}{\psi}_p(y,r)\overadd{1}{\psi}(s,y)\,dy
    +\int_s^r\overadd{i,j-1}{\psi}_p(y,r)\overadd{1,1}{\psi}_p(s,y)\,dy
    \,,
    \qquad 1<j<i+1
\\
    \overadd{i+1,i+1}{\psi}_p(s,r)
    &=
    \int_s^r\overadd{i,i}{\psi}_p(y,r)\overadd{1,1}{\psi}_p(s,y)\,dy
    \,,
\end{align}



% second term contributions to \eqref{4VIII22.w1}:
%  %
%          \begin{align}
%        \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k \partial_u\hBo_{AB}
%        =&
%        \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k \bigg[ \overadd{1}{\Psi}_{AB}(r,u, x^A)
%       	+\overadd{1,0,0}{\psi}(r) \hBo_{AB}|_r
%       	+\overadd{1,0,1}{\psi}(r) P \hBo_{AB}|_r
%       	\nonumber
%       \\
%       &
%       	+\overadd{1,1,0}{\psi}(r)\partial_r \hBo_{AB}|_r
%          +\int_{r_1}^{r} \Big(\overadd{1}{\psi}(s,y) h_{AB}|_s
%        +
%        \overadd{1,1}{\psi}_p(s,r)P h_{AB}|_s
%        \Big)\,
%          ds
%        \bigg]
%        \nonumber
%  \end{align}

%  \begin{align}
%       1. \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k \bigg(
%       	\overadd{1,0,0}{\psi}(r) \hBo_{AB}|_r\bigg)
%       	= &
%       	 \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^k
%       	 \sum_{m=0}^j\binom{j}{m}\partial_r^m\big(\hBo_{AB}\big)\partial^{j-m}_r\overadd{1,0,0}{\psi}(r)
%       	 \nonumber
% \\
%       	= &
%       	\sum_{m=0}^i \sum_{k=0}^i \sum_{j=m}^i
%       	\binom{j}{m} \overadd{i,j,k}{\psi}(r)\partial^{j-m}_r(\overadd{1,0,0}{\psi}(r))
%       	\partial_r^m\big(P^k \hBo_{AB}\big)
%  \end{align}

%  \begin{align}
%     2.   \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k \bigg(
%       	\overadd{1,0,1}{\psi}(r) P\hBo_{AB}|_r\bigg)
%       	= &
%       	 \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^{k+1}
%       	 \sum_{m=0}^j\binom{j}{m}\partial_r^m\big(\hBo_{AB}\big)\partial^{j-m}_r\overadd{1,0,1}{\psi}(r)
%       	 \nonumber
%       	 \\
%       	= &
%       	\sum_{m=0}^i \sum_{k=1}^{i+1} \sum_{j=m}^i
%       	\binom{j}{m} \overadd{i,j,k-1}{\psi}(r)\partial^{j-m}_r(\overadd{1,0,1}{\psi}(r))
%       	\partial_r^m\big(P^{k} \hBo_{AB}\big)
%  \end{align}

%  \begin{align}
%     3.   \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k \bigg(
%       	\overadd{1,1,0}{\psi}(r) \partial_r\hBo_{AB}|_r\bigg)
%       	= &
%       	 \sum_{j=0}^{i}\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^k
%       	 \sum_{m=1}^{j+1}\binom{j}{m-1}\partial_r^{m}\big(\hBo_{AB}\big)\partial^{j-m+1}_r\overadd{1,1,0}{\psi}(r)
%       	 \nonumber
%       	 \\
%       	= &
%       	\sum_{m=1}^{i+1} \sum_{k=0}^i \sum_{j=m-1}^i
%       	\binom{j}{m-1} \overadd{i,j,k}{\psi}(r)\partial^{j-m+1}_r(\overadd{1,1,0}{\psi}(r))
%       	\partial_r^m\big(P^k \hBo_{AB}\big)
%  \end{align}

%   4:
%  \begin{align}
%    \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      & = \sum_{k=0}^i \overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^{j-1} P^k
%       \Big(\overadd{1}{\psi}(r,r) h_{AB}|_r\Big)
%      \nonumber
%      \\
%      & =
%      \sum_{k=0}^i \overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)
%      \sum_{m=0}^{j-1} \binom{j-1}{m}
%       P^k
%       \partial_r^{j-1-m}\Big(\overadd{1}{\psi}(r,r)\Big) \partial_r^{m} h_{AB}|_r
%       \nonumber
%      \\
%      & =
%      \sum_{k=0}^i \overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+\sum_{j=0}^{i-1}\sum_{k=0}^i\sum_{m=j+1}^{i}\binom{m-1}{j}\overadd{i,m,k}{\psi}(r)
%       P^k
%       \partial_r^{m-1-j}\Big(\overadd{1}{\psi}(r,r)\Big) \partial_r^{j} h_{AB}|_r
%  \end{align}
%  %%%%%%%%
 
%  \green{ \begin{align}
%    &\sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%          \nonumber
% \\
%      & = \sum_{k=0}^i \overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
% \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^k\bigg[
%      \sum_{\ell=1}^j
%      \partial_r^{j-\ell}\bigg(\partial^{\ell-1}_x(\overadd{1}{\psi}(r,x))|_{x=r} \hBo_{AB}|_r\bigg)
%       +\int_{r_0}^r \partial_r^j\overadd{1,0}{\psi}(s,r)\hBo_{AB}|s\ds\bigg]
%      \nonumber
% \\
%      & =
%     \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^k\int_{r_0}^r \partial_r^j\overadd{1,0}{\psi}(s,r)\hBo_{AB}|s\ds
%      \nonumber
% \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^k
%      \sum_{\ell=1}^j
%      \partial_r^{j-\ell}\bigg(\partial^{\ell-1}_x(\overadd{1}{\psi}(r,x))|_{x=r} \hBo_{AB}|_r\bigg)
%  \end{align}
%  %
%  }
%  \newpage
%  5:
%  \begin{align}
%     \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^k
%      \int_{r_1}^{r}\overadd{1,1}{\psi}_p(s,r)P h_{AB}|_s\,
%          ds
%      & =
%      \sum_{k=0}^i\overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1,1}{\psi}_p(s,r)P h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^{j-1} P^{k+1}
%       \Big(\overadd{1,1}{\psi}_p(r,r) h_{AB}|_r\Big)
%      \nonumber
%      \\
%      & =
%      \sum_{k=0}^i\overadd{i,0,k}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1,1}{\psi}_p(s,r)P h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+
%      \sum_{j=1}^i\sum_{k=1}^{i+1}\overadd{i,j,k-1}{\psi}(r)
%      \sum_{m=0}^{j-1} \binom{j-1}{m}
%       P^k
%       \partial_r^{j-1-m}\Big(\overadd{1,1}{\psi}_p(r,r)\Big) \partial_r^{m} h_{AB}|_r
%       \nonumber
%      \\
%      & =
%      \sum_{k=1}^{i+1}\overadd{i,0,k-1}{\psi}(r) P^k
%      \int_{r_1}^{r}\overadd{1,1}{\psi}_p(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
%      \\
%      &+
%      \sum_{j=0}^{i-1}\sum_{k=1}^{i+1}\sum_{m=j+1}^{i}\binom{m-1}{j}\overadd{i,m,k-1}{\psi}(r)
%       P^k
%       \partial_r^{m-1-j}\Big(\overadd{1,1}{\psi}_p(r,r)\Big) \partial_r^{j} h_{AB}|_r
%  \end{align}
%  %
%  \green{corrections to 5:}
%  %
%  \begin{align}
%    &\sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)\partial_r^j P^{k+1}
%      \int_{r_1}^{r}\overadd{1,1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%          \nonumber
% \\
%      & = \sum_{k=0}^i \overadd{i,0,k}{\psi}(r) P^{k+1}
%      \int_{r_1}^{r}\overadd{1,1}{\psi}(s,r) h_{AB}|_s\,
%          ds
%      \nonumber
% \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^{k+1}\bigg[
%      \sum_{\ell=1}^j
%      \partial_r^{j-\ell}\bigg(\partial^{\ell-1}_x(\overadd{1,1}{\psi}(r,x))|_{x=r} \hBo_{AB}|_r\bigg)
%       +\int_{r_0}^r \partial_r^j\overadd{1,1}{\psi}(s,r)\hBo_{AB}|s\ds\bigg]
%      \nonumber
% \\
%      & =
%     \sum_{j=0}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^{k+1}\int_{r_0}^r \partial_r^j\overadd{1,1}{\psi}(s,r)\hBo_{AB}|s\ds
%      \nonumber
% \\
%      &+\sum_{j=1}^i\sum_{k=0}^i\overadd{i,j,k}{\psi}(r)P^{k+1}
%      \sum_{\ell=1}^j
%      \partial_r^{j-\ell}\bigg(\partial^{\ell-1}_x(\overadd{1,1}{\psi}(r,x))|_{x=r} \hBo_{AB}|_r\bigg)
%  \end{align}
%  %

% \newpage
% Contributions from 3rd term:
% %
%  \begin{align}
%      \int_{r_1}^{r}
%        \overadd{i}{\psi}(s,r) \partial_u \hBo_{AB}\,ds &=
%        \int_{r_1}^{r}
%        \overadd{i}{\psi}(s,r)
%        \bigg[
%        \overadd{1}{\Psi}_{AB}(s,u, x^A)
%       	+\overadd{1,0,0}{\psi}(s) \hBo_{AB}|_s
%       	+\overadd{1,0,1}{\psi}(s) P \hBo_{AB}|_s
%       	\nonumber
%       \\
%       &
%       	+\overadd{1,1,0}{\psi}(s)\partial_s \hBo_{AB}|_s
%          +\int_{r_1}^{s} \Big(\overadd{1}{\psi}(y,s) h_{AB}|_y
%        +
%        \overadd{1,1}{\psi}_p(y,s)P h_{AB}|_y
%        \Big)\,
%          dy
%        \bigg]\,ds
%  \end{align}
%  %
 
% Contributions from 4th term:
% %
%  \begin{align}
%       \int_{r_1}^{r}
%        \sum_{j=1}^i
%        \overadd{i,j}{\psi}_p(s,r)P^j \partial_u \hBo_{AB}
%          ds
%          &=
%          \int_{r_1}^{r}
%        \sum_{j=1}^i
%        \overadd{i,j}{\psi}_p(s,r)P^j
%          \bigg[
%        \overadd{1}{\Psi}_{AB}(s,u, x^A)
%       	+\overadd{1,0,0}{\psi}(s) \hBo_{AB}|_s
%       	+\overadd{1,0,1}{\psi}(s) P \hBo_{AB}|_s
%       	\nonumber
%       \\
%       &
%       	+\overadd{1,1,0}{\psi}(s)\partial_s \hBo_{AB}|_s
%          +\int_{r_1}^{s} \Big(\overadd{1}{\psi}(y,s) h_{AB}|_y
%        +
%        \overadd{1,1}{\psi}_p(y,s)P h_{AB}|_y
%        \Big)\,
%          dy
%        \bigg]\,ds
%  \end{align}
% %End of Workings /////////////////////////////


==> C2strategy.tex <==
\subsection{Strategy for $C^2$-gluing}
 \label{C2ss10IX22.1}

\ptcr{some duplicate stuff has to be removed; alternatively, do first $C^2$ and then the general case?
we should adapt this as the last steps after the iteration}

{\redca{9X, but should we do it for any k?}
The above argument has been streamlined for an iteration which gives a smooth gluing together with $k$ transverse derivatives  for any finite $k$.
We expect that the scheme is optimal, as a unique solution is obtained.
 \ptcr{is it? if not we should find a unique?}
However,   the last obstructions appearing in that scheme, essential to continue the iteration, can be side-stepped by modifying the last step of the argument. We illustrate this in the case of the $C^2$-gluing. Here
}
the starting point is identical:  the smooth solution on $\mcN_{(r_0,r_1]}$ is extended to one on $\mcN_{(r_0,r_2]}$ using a smooth interpolating field $ \interph $ and smooth gauge fields $\kzeta{1}$ and $\kzeta{2}$ as in \eqref{16III22.2}, with the $u$-derivatives extended as described in Section~\eqref{sec:28VII22.2}. The rest of the argument is a variation of the one in Section~\eqref{ss10IX22.1}, as follows:

\begin{enumerate}
  \item We continue to use  the gauge $\partial_u^i h_{ur}|_\mcN \equiv 0$, $i\in \N$, which guarantees both smoothness of $h_{ur}$ and the validity of  the equations, for all $i$,
%
\begin{eqnarray}
0
   &  = &
  \partial_u^i \delta \red{\mcE}_{rr}  |_\mcN
  \equiv
  - \partial_u^i \delta \red{\mcE}^u{}_{r}  |_\mcN
  \equiv
  \partial_u^i \delta \red{\mcE}^{uu}  |_\mcN
   \,.
   \label{C230IX22.11}
\end{eqnarray}
%
%

      \item  We determine the  gauge field $\kxi 2_A^{\red{[\ge 2]}}$ (equivalently, $\kxi 2^A $ up to the addition
       of a conformal Killing vector field), by matching the pointwise radial charges $\kQ{3,1}{A}^{\red{[\ge 2]}}$ (cf. \eqref{9IX22.11} and \eqref{26IX22.21})
at
 $\tilde\secN_2$. This, together with the gauge conditions $\partial_u^i h_{ur}=0$,  determines the gauge fields $(\partial_u\kxi{2} ^u)^{[\ge 2]}$.



  \item  We determine  the   gauge fields $\kxi{2}^{u[\geq 2]}$ so that  the pointwise radial charges $\chi^{[\geq 2]}$ defined in \eqref{24IX22.2} are continuous
       \ptc{4 obstructions here, probably energy momentum, radial charge Q2}
       at
       $\tilde\secN_2$.

%
  \item The continuity at $r_2$ of the  field $\partial_r h_{uA}$ is achieved using  the  field $\kphi{1}_{AB}$
       \ptc{six obstructions here, radial charge Q1}.
      %

  \item
  \label{step6X22.w5}
  We glue the field  $  h_{uA}$ using   the  field
       $\kphi{4 }_{AB}$ and $\partial_u\kxi{2}^{A[=1]}$.
        This guarantees a continuous
       (and hence smooth, in view of point 4 and the equation satisfied by $h_{uA}$)
       extension of  $ h_{uA}$ across $\{r=r_2\}$, as well as
      %
      \begin{equation}\label{C230IX22.24}
          \delta \red{\mcE}_{rA}|_{\blue{\mcN}}  \equiv -  \delta \red{\mcE}^u{} _{A}|_{\blue{\mcN}} = 0
         \,.
      \end{equation}
     It follows that we have on $\mcN$
    %
    \begin{equation}
        \delta\mcE^A{}_B = g^{AC}\delta \mcE_{CB}
         \,,
        \label{4X22.8}
    \end{equation}
    %

\ptcheck{20X;it looks like identical to the previous scheme with zero $u$ derivatives at each step so far; changes start here}

      \item
      \label{step6X22.w6}
       \ptcheck{20X; this was Step \ref{step5X22.8} before, interchanged with the next one, and the order does not seem to matter for these two}
      The field  $\hBo_{uu}$  is obtained from the conservation condition $\partial_r \chi = 0$ and the fact that $\chi$ has been made continuous by a choice of gauge and by the hypothesis of conservation of $\kQ{2}{}$. This guarantees that the equation
      %
      \begin{equation}\label{C230IX22.21}
         \delta \red{\mcE}_{ru} + \frac 1{2r}
  \zspaceD ^A \delta \red{\mcE}_{rA}  = 0
      \end{equation}
      %
      holds on $\mcN $. It thus follows from \eqref{C230IX22.24} that
      %
      \begin{equation}\label{C230IX22.21b}
         \delta \red{\mcE}_{ru}\big|_{\blue{\mcN}}   = 0 = \delta \red{\mcE}^r{}_{r}\big|_{\blue{\mcN}}\,.
      \end{equation}
      %


  \item
  \label{step6X22.w7}
  \ptcheck{20X; was step \eqref{step5X22.7} before}
   The field  $\partial_u\hBo_{AB}$  is obtained from the conservation condition $\partial_r \kQ{3,1}{A} = 0$ and the fact that $\kQ{3,1}{A}$ has been made continuous by a choice of gauge and by the hypothesis of conservation of $\kQ{1}{}$. This ensures  that the equation
%
\begin{equation}\label{C228IX22.6wr}
\zspaceD^A \big[
  \TS\big(
    \delta \red{\mcE}_{AB}  - \frac{1}{2r^2 }\zspaceD_A \ \delta \red{\mcE}_{rB}
    \big)
  \big]
   =0
\end{equation}
%
holds on $\mcN $. On $S^2$ this implies
 \ptc{watch out for other topologies here}
%
\begin{equation}\label{C22X22.21}
  \TS\big( \delta \red{\mcE}_{AB}  - \frac{1}{2r^2 }\zspaceD_A  \delta \red{\mcE}_{rB}
    \big)
  \big|_\mcN
   =0
    \,.
\end{equation}
%
    This, together with \eqref{C230IX22.24}, guarantees that
      %
      \begin{equation}\label{C230IX22.23}
  \TS\big(
 \delta \red{\mcE}_{AB}
    \big)
   \big|_\mcN   = 0
      \end{equation}
      %


        The divergence identity \eqref{27IX22.2asdf} with $\nu = r$ reads
%
\begin{equation}\label{C21X22.5}
 0\equiv \partial_u  \delta  \red{\mcE}^u{}_r
   +
   \frac{1}{r^2} \partial_r  (r^2  \delta  \red{\mcE}^r{}_r )
   +   \frac{1}{\sqrt{|\det \zgamma |}} \partial_A (\sqrt{|\det \zgamma |} \delta  \red{\mcE}^A{}_r )
   -
   \frac{1}{r}
        g^{AB}
    \delta \red{\mcE}_{AB}
   \,,
\end{equation}
%
so that, in view of \eqref{C230IX22.11}, \eqref{C230IX22.24} and \eqref{C230IX22.21b}, we have now
%
\begin{equation}\label{C21X22.6}
 0 =
   \frac{1}{r}
        g^{AB}
     \delta \red{\mcE}_{AB}
        \big|_{\blue{\mcN}}
   \,.
\end{equation}
%
Together with \eqref{4X22.8}, we have thus
%
\begin{equation}\label{C22X22.4}
   \delta \red{\mcE}_{AB}
  \big|_{\blue{\mcN}}
   =0 = \delta \red{\mcE}^A{}_{B}
  \big|_{\blue{\mcN}}
    \,.
\end{equation}
%
    \item
    \label{step6X22.w8}
   The gauge field $\partial^2_u \kxi{2}^A$ and the field
       $\kphi{5}_{AB}$ are chosen to ensure a continuous extension of  $\partial_u h_{uA}$ across $\{r=r_2\}$, as well as
      %
      \begin{equation}\label{C230IX22.24ag}
         \partial_u \delta \red{\mcE}_{rA}|_{\blue{\mcN_{[r_0,r_2)}}}  \equiv -\partial_u \delta \red{\mcE}^u{} _{A}|_{\blue{\mcN_{[r_0,r_2)}}} = 0
         \,.
      \end{equation}
      %
       It follows that we have on $\mcN_{[r_0,r_2)}$,
    %
    \begin{equation}
        \delta\partial_u\mcE^A{}_B|_{\blue{\mcN_{[r_0,r_2)}}} = \delta g^{AC}\partial_u\mcE_{CB}|_{\blue{\mcN_{[r_0,r_2)}}}\,.
        \label{4X22.8ii}
    \end{equation}
    %
      Further, the divergence identity gives
%
\begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \red{\mcE}^{\mu}{}_A
    \nonumber
\\
 &= &
 r^{-2}\partial_r(r^2  \delta \red{\mcE}^r{}_A)
   + \partial_u \delta \red{\mcE}^u{}_A
    + \zspaceD_B \delta \red{\mcE}^B{}_A
 \,.
 \label{C22X22.6}
\end{eqnarray}
%
The identity \eqref{C22X22.6} together with \eqref{C230IX22.24},  \eqref{C22X22.4} and \eqref{C230IX22.24ag} gives
%
\begin{eqnarray}
  0 & =  &
  r^{-2}\partial_r(r^2  \delta \red{\mcE}^r{}_A)
    \Big|_{\blue{\mcN_{[r_0,r_2)}}}
 \,.
  \label{C21X22.3}
\end{eqnarray}
%
Continuity at $r_1$, where all the fields $
    \red{\mcE}_{\mu\nu} $ vanish, shows that
%
\begin{equation}
     \delta \red{\mcE}^r{}_A  |_{\blue{\mcN_{[r_0,r_2)}}}=0 =
      \delta \red{\mcE}_{uA} |_{\blue{\mcN_{[r_0,r_2)}}}
    \,.
     \label{C22X22.8}
\end{equation}
%
        \item  The explicit form \eqref{9XI20.t1} of the equation $ \delta \red{\mcE}_{uA} =0$ together with the continuity of $\hBo_{uu}$ (Step \ref{step6X22.w6}), $\hBo_{uA}$ (Step \ref{step6X22.w5})  and $\partial_u\hBo_{AB}$ (Step \ref{step6X22.w7}) at $r_2$ ensures the continuity of $\partial_r\partial_u\hBo_{uA}$ at $r_2$. Further, it follows from \eqref{6X22.w1} and \eqref{6X22.w6} with $i=1$ that
%
        \begin{equation}
            \label{6X22.w2}
    \partial_r\kQ{1,1}{}\big|_{\mcN} =
    %0\,,\qquad
            \partial_r \kQ{3,2}{A}^{[=1]}\big|_{\mcN} = 0\,.
        \end{equation}
%
 \ptcr{I need to continue carefully from here on, 21X22}
    \item
    \label{step6X22.w10}
    We construct the field $\partial_u \hBo_{uu}$ on $\mcN_{[r_1,r_2)}$ by enforcing there the equation
            %
      \begin{equation}\label{C21X22.1}
         \delta  \partial_u\red{\mcE}_{ru} + \frac 1{2r}
  \zspaceD ^A  \delta \partial_u\red{\mcE}_{rA}  = 0\,.
      \end{equation}
      %
     Equivalently,
       $\partial_r \kochi{1} =0$, i.e.\ (compare \eqref{24IX22.2})
    %
    \begin{equation}
         r  \partial_u\hBo_{uu}
         - \big(  \frac{ r}{2}\partial_r  \zspaceD^A   \partial_u h_{uA}
       -\frac{1}{2r}  \zspaceD^A\zspaceD^B  \partial_u h_{AB}
       \big) =
         \kochi{1}[\dt_{\secN_1}]\,.
    \end{equation}
      %
      It follows from \eqref{C21X22.1} and \eqref{C230IX22.24ag} that
      %
      \begin{equation}\label{C23X22.2}
         -\delta  \partial_u\red{\mcE}^u{}_{u}|_{\mcN_{[r_1,r_2)}}
         \equiv
         \delta  \partial_u\red{\mcE}_{ru}|_{\mcN_{[r_1,r_2)}} = 0\,.
      \end{equation}
      %
      The divergence identity gives now
      %
    \begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \red{\mcE}^{\mu}{}_u
    \nonumber
\\
 &= &
 r^{-2}\partial_r(r^2  \delta \red{\mcE}^r{}_u)
   + \partial_u \delta \red{\mcE}^u{}_u
    + \zspaceD_B \delta \red{\mcE}^B{}_u
 \,,
 \label{C22X22.6b}
\end{eqnarray}
%
while we note that \eqref{C230IX22.21b} and \eqref{C22X22.8}  gives
%
    \begin{equation}
        \label{C24X22.1}
        \mcE^r{}_u|_{\blue{\mcN_{[r_0,r_2)}}} = -\mcE_{uu}|_{\blue{\mcN_{[r_0,r_2)}}}\,, \qquad \mcE^A{}_u|_{\blue{\mcN_{[r_0,r_2)}}} = 0\,.
    \end{equation}
    %
   It follows from \eqref{C24X22.1} and \eqref{C23X22.2} that the divergence identity \eqref{C22X22.6b} becomes
          %
    \begin{eqnarray}
  0
 &= &
 -r^{-2}\partial_r(r^2  \delta \red{\mcE}_{uu})|_{\blue{\mcN_{[r_0,r_2)}}}
 \,.
 \label{C22X22.62}
\end{eqnarray}
%
Continuity and vanishing at $r_1$ implies that
%
\begin{equation}\label{C22X22.7}
    \delta \red{\mcE}_{uu}
    \big |_{\mcN_{[r_1,r_2)}}=0
\end{equation}
%
The explicit form \eqref{13VIII20.t3} of \eqref{C22X22.7}, together with the continuity of $\hBo_{uu}$ (Step 6), $\hBo_{uA}$ (Step 5), $\partial_u \hBo_{uA}$ (Step 8)  and $\partial_u \hBo_{AB}$ at $r_2$ (Step 7), ensures the continuity of $\partial_u\hBo_{uu}$ at $r_2$.
     %
     \item
     \label{step6X22.w11}
    We determine the  gauge field $\partial_u\kxi 2^{A\red{[\ge 2]}}$ by matching the radial charge $\kQ{3,2}{A}^{\red{[\ge 2]}}$ (cf. \eqref{9IX22.11} and \eqref{9IX22.9}) at $r_2$ with the value at $r_1$. This, together with the gauge conditions $\partial_u^i h_{ur}=0$,  determines the gauge fields $\partial_u^{2}\kxi{2} ^u$.
\item
\label{step6X22.w12}
   The  field $\partial^2_u\hBo_{AB}$ on $\mcN_{[r_1,r_2)}$ is obtained by the condition  $ \partial_r \kQ{3,2}{A}=0 $ . Continuity at $r_2$ follows from the continuity of $\kQ{3,2}{A}$ there.  This  ensures  that the equation
%
\begin{equation}\label{C228IX22.6wrii}
\zspaceD^A \big[
  \TS\big(
    \delta \partial_u\red{\mcE}_{AB}  - \frac{1}{2r^2 }\zspaceD_A \delta \partial_u\red{\mcE}_{rB}
    \big)
  \big]
   =0
\end{equation}
%
holds on $\mcN $. On $S^2$ this implies
 \ptc{watch out for other topologies here}
%
\begin{equation}\label{C22X22.21ii}
  \TS\big( \delta \partial_u\red{\mcE}_{AB}  - \frac{1}{2r^2 }\zspaceD_A  \delta \partial_u\red{\mcE}_{rB}
    \big)
  \big|_\mcN
   =0
    \,.
\end{equation}
%
 It now follows from \eqref{C230IX22.24ag} that
 \ptc{watch out for other topologies here}
%
\begin{equation}\label{C22X22.3ii}
  \TS\big(
   \delta \partial_u \red{\mcE}_{AB}
    \big)
  \big|_{\blue{\mcN_{[r_0,r_2)}}}
   =0
    \,.
\end{equation}
%

The $u$ differentiated divergence identity \eqref{27IX22.2asdf} with $\nu = r$ reads
%
\begin{equation}\label{C21X22.5ii}
 0\equiv \partial^2_u  \delta  \red{\mcE}^u{}_r
   +
   \frac{1}{r^2} \partial_r  (r^2  \delta  \partial_u\red{\mcE}^r{}_r )
   +   \frac{1}{\sqrt{|\det \zgamma |}} \partial_A (\sqrt{|\det \zgamma |} \delta  \partial_u\red{\mcE}^A{}_r )
   -
   \frac{1}{r}
        g^{AB}
    \delta \partial_u\red{\mcE}_{AB}
   \,,
\end{equation}
%
so that, in view of \eqref{C230IX22.11}, \eqref{C230IX22.24ag}, \eqref{C23X22.2} and \eqref{C22X22.3ii}, we have now
%
\begin{equation}\label{C21X22.6ii}
 0 =
   \frac{1}{r}
        g^{AB}
     \delta \partial_u\red{\mcE}_{AB}
        \big|_{\blue{\mcN_{[r_0,r_2)}}}
   \,.
\end{equation}
%
Together with \eqref{C22X22.3ii} and \eqref{4X22.8ii}, it follows that
 \ptc{watch out for other topologies here}
%
\begin{equation}\label{C22X22.4ii}
  \delta \partial_u\red{\mcE}_{AB}
  \big|_{\blue{\mcN_{[r_0,r_2)}}}=0=\delta \partial_u\red{\mcE}^A{}_{B}
  \big|_{\blue{\mcN_{[r_0,r_2)}}}
    \,.
\end{equation}
%
    \item
    \label{step6X22.w13}
    We glue the field $\partial^2_u h_{uA}$ using the gauge field $\partial^3_u \kxi{2}^A$ and the field
       $\kphi{6}_{AB}$ to ensure a continuous extension of  $\partial^2_u h_{uA}$ across $\{r=r_2\}$, as well as
      %
      \begin{equation}\label{C230IX22.24ii}
         \partial^2_u \delta \red{\mcE}_{rA}|_{\blue{\mcN_{[r_0,r_2)}}}  \equiv -\partial^2_u \delta \red{\mcE}^u{} _{A}|_{\blue{\mcN_{[r_0,r_2)}}} = 0
         \,.
      \end{equation}
      %
      Further, the $u$-differentiated divergence identity gives
%
\begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \partial_u\red{\mcE}^{\mu}{}_A
    \nonumber
\\
 &= &
 r^{-2}\partial_r(r^2  \delta\partial_u \red{\mcE}^r{}_A)
   + \partial^2_u \delta \red{\mcE}^u{}_A
    + \zspaceD_B \delta \partial_u\red{\mcE}^B{}_A
 \,.
 \label{C22X22.6ii}
\end{eqnarray}
%
The identity \eqref{C22X22.6ii} together with \eqref{C230IX22.24ii} and \eqref{C22X22.4ii} gives
%
\begin{eqnarray}
  0 & =  &
  r^{-2}\partial_r(r^2  \delta \partial_u \red{\mcE}^r{}_A)
    \Big|_{\blue{\mcN_{[r_0,r_2)}}}
 \,.
  \label{C21X22.3ii}
\end{eqnarray}
%
Continuity at $r_1$, where all the fields $
   \partial_u^i  \red{\mcE}_{\mu\nu} $ vanish, shows that
%
\begin{equation}
     \delta \partial_u\red{\mcE}^r{}_A  |_{\blue{\mcN_{[r_0,r_2)}}}=0 =
      \delta \partial_u\red{\mcE}_{uA} |_{\blue{\mcN_{[r_0,r_2)}}}
    \,.
     \label{C22X22.8ii}
\end{equation}
%
        \item
         Differentiation of \eqref{9XI20.t1} gives
%
    \begin{eqnarray}
    r^{2}\partial_{r}\partial_u\left(\frac{\partial_u h_{uA}}{r^{2}}\right) & = &
    -\frac{1}{ r^2} \Big[
    \zspaceD^{B}\zspaceD_{A}\partial_u{h}_{uB}
    -\zspaceD^{B}\zspaceD_{B}\partial_u{h}_{uA}
    + \zspaceD^{B}\partial^2_u{h}_{A B}
    \nonumber
    \\
    &&
    -r^{2}\Big(
    \left(\twoscsign-r^{2}\alpha^{2}\right)\partial_{r}^{2}\partial_uh_{uA}
    + 2\alpha^{2}\partial_u h_{uA}
 + \partial_{r}\zspaceD_{A}{\partial_u h}_{uu}
        \Big)\Big]
    \,.
 \phantom{xxxxx}
    \label{C29XI20.t1cii}
    \end{eqnarray}
    %
        The explicit form \eqref{C29XI20.t1cii} of the equation $ \delta\partial_u \red{\mcE}_{uA} =0$ together with the continuity of $\partial_u\hBo_{uu}$ (Step \ref{step6X22.w10}), $\partial_u\hBo_{uA}$ (Step \ref{step6X22.w13})  and $\partial^2_u\hBo_{AB}$ at $r_2$ (Step \ref{step6X22.w12}) ensures the continuity of $\partial_r\partial^2_u\hBo_{uA}$ at $r_2$.
    \item
    We construct the field $\partial^2_u \hBo_{uu}$ on $\mcN_{[r_1,r_2)}$ by enforcing there the equation
            %
      \begin{equation}\label{C21X22.1ii}
         \delta  \partial^2_u\red{\mcE}_{ru} + \frac 1{2r}
  \zspaceD ^A  \delta \partial^2_u\red{\mcE}_{rA}  = 0\,.
      \end{equation}
      %
     Equivalently,
       $\partial_r \kochi{2} =0$, i.e.\ (compare \eqref{24IX22.2})
    %
    \begin{equation}
         r  \partial^2_u\hBo_{uu}
         - \big(  \frac{ r}{2}\partial_r  \zspaceD^A   \partial^2_u h_{uA}
       -\frac{1}{2r}  \zspaceD^A\zspaceD^B  \partial^2_u h_{AB}
       \big) =
         \kochi{2}[\dt_{\secN_1}]\,.
    \end{equation}
      %
      It follows from \eqref{C21X22.1ii} and \eqref{C230IX22.24ii} that
      %
      \begin{equation}\label{C23X22.2ii}
         -\delta  \partial^2_u\red{\mcE}^u{}_{u}|_{\mcN_{[r_1,r_2)}} =
         \delta  \partial^2_u\red{\mcE}_{ru}|_{\mcN_{[r_1,r_2)}} = 0\,.
      \end{equation}
      %
      Further, the $u$-differentiated divergence identity reads
      %
    \begin{eqnarray}
  0 &\equiv & \nabla_\mu \delta \partial_u \red{\mcE}^{\mu}{}_u
    \nonumber
\\
 &= &
 r^{-2}\partial_r(r^2  \delta \partial_u \red{\mcE}^r{}_u)
   +  \delta\partial^2_u  \red{\mcE}^u{}_u
    + \zspaceD_B \delta \partial_u \red{\mcE}^B{}_u
 \,,
 \label{C22X22.6bii}
\end{eqnarray}
Meanwhile, \eqref{C23X22.2} and \eqref{C22X22.8ii} gives
%
    \begin{equation}
        \label{C24X22.1ii}
        \partial_u\mcE^r{}_u|_{\blue{\mcN_{[r_0,r_2)}}} = -\partial_u\mcE_{uu}|_{\blue{\mcN_{[r_0,r_2)}}}\,, \qquad \partial_u\mcE^A{}_u|_{\blue{\mcN_{[r_0,r_2)}}} = 0\,.
    \end{equation}
    %
   It follows from \eqref{C24X22.1ii} and \eqref{C23X22.2ii} that the divergence identity \eqref{C22X22.6bii} becomes
          %
    \begin{eqnarray}
  0
 &= &
 -r^{-2}\partial_r(r^2  \delta \partial_u\red{\mcE}_{uu})|_{\blue{\mcN_{[r_0,r_2)}}}
 \,.
 \label{C22X22.62ii}
\end{eqnarray}
%
Continuity and vanishing at $r_1$ implies that
%
\begin{equation}\label{C22X22.7ii}
    \delta \partial_u \red{\mcE}_{uu}
    \big |_{\mcN_{[r_1,r_2)}}=0
\end{equation}
%
We can now invoke the $u$-differentiated version of  \eqref{13VIII20.t3},
%
\begin{eqnarray}
  0 & = &  \partial_u \delta \red{\mcE}_{uu}
    \big |_{\mcN_{[r_1,r_2)}}
  \nonumber
\\
 & = &     \frac{1}{ r^2}\Big[2\Big(
      \partial_{u}
    +(\red{\alpha^2} r^2-\twoscsign) \partial_{r}
    -\frac{1}{r}
    \Big) \zspaceD^{A} \partial_u {h}_{u A}
    -  \zspaceD^{A} \zspaceD_{A} \partial_u {h}_{u u}
     \nonumber \\
&&
-(\red{\alpha^2} r^2-\twoscsign) \Big(\frac{\zspaceD^{A} \zspaceD^{B} \partial_u {h}_{A B}}{r^2}\Big)
-2 r \partial_{u} ^{2}{h}_{u u}
-2 (\red{\alpha^2} r^2-\twoscsign) \partial_{r}(r \partial_u {h}_{u u})
\Big]
\, . \phantom{xxxxx}
\label{C213VIII20.t3rs}
\end{eqnarray}
%
 The  continuity of $\partial_u \hBo_{uu}$, $\partial^2_u \hBo_{uA}$  and $\partial_u \hBo_{AB}$ at $r_2$ ensures continuity of $\partial_u^2\hBo_{uu}$ at $r_2$.
\end{enumerate}


We now pass to the details of the above. 

==> CKV.tex <==
\section{Conformal Killing vectors on compact Einstein manifolds}
 \label{App30X22}
 \newcommand{\ddim}{{\blue{d}}}
 \newcommand{\dmanif}{\blue{{}^dM}}
 \newcommand{\dmetric}{{\blue{\mathring{\gamma}}}}
 \newcommand{\dnabla}{\blue{\mathring{D}}}
 \newcommand{\dDelta}{\blue{\Delta_{\dmetric}}}
 \newcommand{\dR}{\blue{\mathring{R}}}

 Consider the conformal Killing equation on a closed $\ddim$-dimensional manifold $(\dmanif,\dmetric)$, with $\ddim \ge 2$:
 %
 \begin{equation}\label{30X22.CKV1}
    \dnabla _A \xi_B +  \dnabla _B \xi_A
    =  \frac2 \ddim \dnabla ^C \xi_C
    \dmetric _{AB}
    \,.
 \end{equation}
 %
Taking the divergence of \eqref{30X22.CKV1}, commuting derivatives, and using \eqref{30X22.CKV2}
one obtains
 %
 \begin{equation}\label{30X22.CKV3}
    \dnabla ^A \dnabla _A \xi_B   + \zR_{BC} \xi^C
    =  \frac {2-d} \ddim \dnabla_A \dnabla ^C \xi_C
    \,.
 \end{equation}
 %
Suppose that $d=2$, then the right-hand side vanishes. Multiplyng by $\xi^B$ and integrating over $\dmanif$ one obtains
 %
 \begin{equation}\label{30X22.CKV4}
   \int ( | \dnabla   \xi|^2    -  \zR_{BC} \xi^B\xi^C
    =  0
    \,.
 \end{equation}
 %
 If $\zR_{BC} < 0$ we find that $\xi \equiv0$. If $\zR_{BC} \le 0$ the only conformal Killing vectors are covariantly constant vector fields.

 Suppose that $\zR_{BC}<0$, and consider the divergence operator $\zdivtwo$ on two-symmetric trace-free tensors,
  \ptcr{this is in dim two for the moment, since we haven't shown that there are CKV's in higher dim yet; but this should follow from the usual theory}
 %
 \begin{equation}\label{30X22.CKV5}
   (\zdivtwo h)_A:= \dnabla^B h_{AB}
   \,.
 \end{equation}
 %
 On a two-dimensional closed negatively curved manifold of genus $g$ the operator $\zdivtwo$ has a $6(g-6)$ dimensional kernel.


 We claim that $\zdivtwo$ is surjective. Indeed, let $\xi$ be $L^2$-orthogonal to its image, then for all smooth tensors $h $ we have
 %
 \begin{equation}\label{30X22.CKV5}
  0 =  \int \xi^A \dnabla^B h_{AB}
  =  - \int \dnabla^B\xi^A  h_{AB} =
   - \int TS(\dnabla^B\xi^A ) h_{AB}
   \,.
 \end{equation}
 %
 This shows that $TS(\dnabla^B\xi^A )=0$, hence $xi^A$ is a conformal vector field. Since no such fields exist, our claim is established.



 Consider, next, the operator $\xi \mapsto C(\xi)$




\reject
\ptcr{not used for the moment, for recycling}
Suppose that  $(\dmanif,\dmetric)$ is Einstein, thus  the Ricci tensor $\dR_{AB}$ of $\dmetric$ satisfies
%
\begin{equation}\label{30X22.CKV2}
  \dR_{AB} = \frac{\dR}{\ddim} \dmetric _{AB}
  \,.
\end{equation}
% 

Commuting derivatives, when $\dR <0$ the equation $\Lop \xi = 0$ (cf.\ \eqref{30X22.31}) implies
%
\begin{equation}\label{30X22}
  \dDelta \dnabla_A \xi^A = 0
  \,,
\end{equation}
%
hence $\dnabla_A \xi^A = 0$.
 \ptcr{so what? guess is: for generic negatively curved manifolds there are no nontrivial solutions} 

==> InconvenientCase.tex <==
\subsubsection{The inconvenient $(n,k)$ case}
\label{ss5IX23.1}

 \ptcheck{28IX23, read the whole section without checking the calculations}

Keeping in mind that the case $m = 0$ has already been covered above, in what follows we consider only the case $m\neq 0$.

In the inconvenient $(n,k)$ case, the equation for $\overadd{p}{\Hf}{}^{[\CKVp]}_{uA}$ in \eqref{11III23.1} and that for $\overadd{p}{q}{}^{[\TTtp]}_{AB}$ in \eqref{11III23.2} may involve $\kphi{i}_{AB}^{[\TTtp]}$'s of the same index $i$. This forces us to consider the $\overadd{p}{\Hf}{}^{[\CKVp]}_{uA}$ and $\overadd{p}{q}{}_{AB}^{[\TTtp]}$ equations together as a system of coupled equations.

First,
 \ptcr{should be already said in the convenient section and here should be as "Recall"?}
 we note that
in the transport equations \eqref{6III23.w11} and \eqref{17IV23.2} for $\overadd{p}{q}_{AB}$, $p\geq \frac{n+1}{2}$, every term involving $\log(r/r_2)$ and $\overadd{p}{\psi}_L$ vanishes, since each of them contains the operator
    %
    $$\ck{-2}{\ofPnoP}\ck{-1}{\ofPnoP} \circ P \,,$$
    %
    which is identically zero when acting on $2$-covariant symmetric, tracefree tensors (cf.\  Appendix \ref{ss13VI.1}).
    Hence, the transport equation for $\overadd{p}{q}_{AB}$ can be written as
    %
\begin{align}
    \partial_r  \overadd{i}{q}_{AB}  &=  \overadd{i}{\psi}\ofP\, r^{(n-7-2i)/2} h_{AB}
    + m^i \overadd{i}{\psi}_{\red{[m]}} r^{\frac{n-7-2i(n-1)}{2}} h_{AB}
    \nonumber
    \\
    &\quad
     + \sum_{j,\ell}^{i_{**}}  m^{j} \overadd{i}{\psi}_{j,0}\ofP\, r^{\frac{n-7}{2} - i -  j (n-2) } h_{AB} \, ,
     \quad 1 \leq i \leq k \,,
    \label{6III23.w6c}
\end{align}
%
with
%
\begin{align}
    \overadd{i}{q}_{AB}&= \partial_u \overadd{i-1}{q}_{AB}
    - \overadd{i-1}{\psi}\ofP \, \qh_{AB}^{(n-5-2i)/2}
    % - \alpha^{2(i-1)} \overadd{i-1}{\psi}_{[\alpha]} \qh_{AB}^{(n-9+2i)/2}
    % \nonumber
    % \\
    % &\quad
    - m^{i-1} \overadd{i-1}{\psi}_{\red{[m]}} \qh^{(\frac{n-7-2(i-1)(n-1)}{2})}_{AB}
    % - \alpha^2 \mathcal{\tilde K}(2(i-1),P)  \overadd{i-2}{q}_{AB}
    \nonumber
    \\
    &\quad
    - \sum_{j,\ell}^{(i-1)_{**}}  m^{j}
    % \alpha^{2\ell}
    \overadd{i-1}{\psi}_{j,0}\ofP \, \qh^{(\frac{1}{2} (n-7- 2 (i-1) - 2 j (n-2)))}_{AB}
    \, ,
     \quad 1 \leq i \leq k \,.
    \label{6III23.w8b}
\end{align}
%
The associated integrated transport equation then reads
%
\begin{align}
    & \underbrace{\overadd{p}{q}_{AB} \big|_{\secN_2} -\overadd{p}{ q}_{AB} \big|_{\secN_1} + \text{known fields}}_{=: \overadd{p}{r}_{AB}}
    \nonumber
    \\
    &=    \text{gauge fields } + \overadd{p}{\psi}\ofP \, \kphit{AB}{(7-n+2p)/2}
    + m^p \overadd{p}{\psi}_{\red{[m]}} \kphit{AB}{(7-n+2p(n-1))/2}
    \nonumber
    \\
    & \quad
    + \sum_{j,\ell}^{p_{**}}  m^{j}
    %\alpha^{2\ell}
    \overadd{p}{\psi}_{j,0}\ofP \, \kphit{AB}{p - \frac{n-7}{2} +  j (n-2) }
    \,,
    \quad  1\leq p\leq k\,,
    \label{22VIII23.2c}
\end{align}
%
where the ``known fields'' on the left-hand side refer to the field $\interph$ and those gauge fields which have been predetermined in Section \ref{s10IX22.1} for the case $m\neq 0$ and $\alpha = 0$; an analysis of the ``gauge fields'' appearing on the right-hand side will be provided below.

For consideration of the coupled system for $\overadd{p}{\Hf}{}^{[\CKVp]}_{uA}$ and $\overadd{p}{q}{}^{[\TTtp]}_{AB}$, it turns out to be convenient to write the interpolating fields $\kphi{p}{}^{[\TTtp]}$ as
%
\begin{align}
\label{8IX23.w3}
    \kphi{p}{}^{[\TTtp]} = C(\TTtpvec{p})
\end{align}
%
where $\TTtpvec{p} \in \CKVp$ is the unique vector solution to \eqref{8IX23.w3} (cf.\  Appendix \ref{ss8IX23.1}). Furthermore, we have the following commutation relation:
    %
    \begin{align}
        \zdivtwo \circ (a P + \TSzlap + 2 \tric + c) \hat\varphi
        =
        (a \zdivtwo \circ C + \TSzlap + (n-2)\myGauss + c) \zdivtwo \hat\varphi\,,
    \end{align}
    %
which allows us to write the divergence of (the $\TTtp$ projection of) \eqref{22VIII23.2c} as
%
\begin{align}
    \underbrace{\zspaceD^A \overadd{p}{r}{}^{[\TTtp]}_{AB}}_{=:  \overadd{p}{r}_B}
    &=    \text{gauge fields } + \overadd{p}{\tilde\psi}\ofDC \circ \zdivtwo\circ C (\TTtpvec{\frac{7-n+2p}{2}})
    \nonumber
    \\
    &\quad
    + m^p \overadd{p}{\psi}_{\red{[m]}} \zdivtwo\circ C (\TTtpvec{\frac{7-n+2p(n-1)}{2}})
    \nonumber
    \\
    & \quad
    + \sum_{j,\ell}^{p_{**}}  m^{j}
    %\alpha^{2\ell}
    \overadd{p}{\tilde\psi}_{j,0}\ofDC \, \zdivtwo\circ C ( \TTtpvec{p - \frac{n-7}{2} +  j (n-2)})
    \,,
    \quad  1\leq p\leq k\,,
    \label{9IX23.w1}
\end{align}
%
where the notation $\tilde{U}\ofP$ (a tilde over an operator $U$) denotes the replacement of all appearances of the operator $P := C\circ\zdivtwo$, respectively   $\tric$, in $U$ by the operator $\zdivtwo\circ C$,  respectively   $(n-2)\myGauss$.
 \ptc{needs checking}
Similarly to the convenient case (cf.\ \eqref{20VIII23.1}),  in order to simplify notation we group terms together and
 rewrite \eqref{9IX23.w1} as
%
\begin{align}
    \overadd{p}{r}_B
    = \text{gauge fields}
    + \sum_{j=\frac{7 - n + 2p}{2}}^{\frac{7-n+2p(n-1)}{2}} \overadd{p}{\tilde\psi}_j \circ \zdivtwo \circ C (\TTtpvec{j} )\,,
    \quad
    1 \leq p \leq k \,,
    \label{9IX23.w2}
\end{align}
%
with some operators $\overadd{p}{\tilde\psi}_j $.
Meanwhile, the integrated transport equation for $\overadd{p}{\Hf}{}^{[\CKVp]}_{uA}$ is as given in \eqref{11III23.1}, which we rewrite as:
%
 \begin{align}
     & \underbrace{
     \big(
      \overadd{p}{\Hf}_{uA}\big|_{\secN_2} - \overadd{p}{\tilde\Hf}_{uA}\big|_{\tilde\secN_1}
      + \text{known fields}
      \big)^{[\CKVp]}}_{ =: \overadd{p}{s}_{A}}
      \nonumber
\\
       &=
       \text{gauge fields} +
       \overadd{p}{\tilde\chi}\ofDC \, \zdivtwo\circ C(\TTtpvec{p+4})
    +  m^p  \overadd{p}{\tilde\chi}_{\red{[m]}} \zdivtwo\circ C(\TTtpvec{p(n-1)+4})
     \nonumber
\\
    & \quad
    + \sum_{\substack{j,\ell,
    \\
    (p + 4) + j (n - 2) >4 }}^{p_*}
    m^{j}  \overadd{p}{\chi}_{j,0}\ofDC \,\zdivtwo\circ C(\TTtpvec{(p + 4) + j (n - 2)})\,,
    \label{19VIII23.2b}
 \end{align}
 %
where, as before, the ``known fields'' on the left-hand side refer to fields which have already been determined up to this point. These include those gauge fields which have been predetermined in section \ref{s10IX22.1} for the case $m\neq 0$ and $\alpha = 0$ and fields $\zspaceD^A \interph_{AB}^{[\TTtp]}$ and $\zspaceD^A \kphi{4}_{AB}^{[\TTtp]}$; this last field is the reason for the exclusion of $(p + 4) + j (n - 2) = 4 $ from the summation. Similar to the convenient case, we rewrite \eqref{19VIII23.2b} as:
 %
 \begin{align}
     \overadd{p}{s}_{A}
       &=
    \sum_{i=5}^{p(n-1)+4}
    \overadd{p}{\tilde\chi}_{i} \circ  \zdivtwo\circ C(\TTtpvec{i})\,.
    \label{20VIII23.1b}
 \end{align}
 %

\input{uvdef}

We can then write the coupled system as follows: we let
%
\begin{align}
u_k &:=  \left\{
           \begin{array}{ll}
(
                \overadd{\frac{n-3}{2}}{r} \,,
                \overadd{1}{r} \,,
               \dots \,,
               \overadd{\frac{n-5}{2}}{r} \,,
               \overadd{1}{s} \,,
               \dots \,,
               \overadd{k}{s}
           )^T, & \hbox{$k=\frac{n-3}{2}$;} \\
(
                \overadd{\frac{n-1}{2}}{r}\,,
                \overadd{\frac{n-3}{2}}{r} \,,
                \overadd{1}{r} \,,
               \dots \,,
               \overadd{\frac{n-5}{2}}{r} \,,
               \overadd{1}{s} \,,
               \dots \,,
               \overadd{k}{s} \,,
               \underbrace{ \overadd{k}{r}  \,,
                 \overadd{k-1}{r}  \,,
                \dots \,,
                 \overadd{\frac{n+1}{2}}{r}}_{k_n \text{ terms}}
           )^T, & \hbox{$k>\frac{n-3}{2}$,}
           \end{array}
         \right.
           \\
 \upsilon_{k} &:=
 \left\{
   \begin{array}{ll}
     (
     \upsilon_{k,2} \,,
 \TTtpvec{\frac{9-n}{2}} \,,
 \dots \,,
 \TTtpvec{1}  \,,
 \TTtpvec{4}  \,,
 \dots \,
 \TTtpvec{4+k}
 )^{T [\CKVp]}, & \hbox{$k=\frac{n-3}{2}$;} \\
     (
      \kxi{2}_A \,,
     \upsilon_{k,2} \,,
 \TTtpvec{\frac{9-n}{2}} \,,
 \dots \,,
 \TTtpvec{1}  \,,
 \TTtpvec{4}  \,,
 \dots \,
 \TTtpvec{4+k} \,,
 \partial^{k_n}_u \kxi{2}_A \,,
 \partial^{k_n-1}_u \kxi{2}_A \,,
 \dots \,,
 \partial_u \kxi{2}_A
 )^{T [\CKVp]}, & \hbox{$k>\frac{n-3}{2}$.}
   \end{array}
 \right.
\end{align}
 %
 where
 %
 \index{$k_n$}
 %
\begin{equation}\label{2X23.1}
 0\le k_n :=\left\{
           \begin{array}{ll}
             0, & \hbox{$k=\frac{n-3}{2}$;} \\
             k-\frac{n-1}{2}, & \hbox{$k\ge \frac{n-1}{2}$.}
           \end{array}
         \right.
\end{equation}
 %
  {\redc
  Note that $u_k$ contains all the $\overadd{j}{r}$'s and  $\overadd{j}{s}$'s, $j\in\{1,\ldots, k\}$, that neither $\overadd{2}{w}{}^{[S]}$ nor  $\overadd{3}{w} $  appear in the list, and that $\overadd{2}{w}{}^{[V]}$ enters through $v_{k,2}$;
   }
   this particular arrangement of terms in the vectors $u_k$ and $v_k$ is convenient for checking the ellipticity of the system.

{\redc
We claim, first, that the system \eqref{9IX23.w2} and \eqref{20VIII23.1b} separates into $V$- and $S$-parts as
 \ptcr{recheck the borderline case k= (n-3)/2}
  \ptcr{is it clear that there is no mixing between the scalar and vector parts?}
%
\begin{align}
    u_k^{\red{[X]}} = \Lambda^{\red{[X]}}_k \upsilon_k^{\red{[X]}} + \mathcal{N}^{\red{[X]}}_k  \rho_k^{\red{[X]}}\,,
    \quad
    X \in \{V,S\}
     \,,
    \label{4IX23.1}
\end{align}
%
where $\Lambda^{\red{[X]}}_k $ is a $2k\times 2k$ matrix of operators, $\mathcal{N}_{k}$ is a $2k \times k(n-2)$ matrix of operators and
%
 \begin{align}
     % \mathcal{N}_k :=
     % \begin{pmatrix}
     % \overadd{\frac{n-1}{2}}{\tilde\psi}_{5+k} & \ldots & \overadd{\frac{n-3}{2}}{\tilde\psi}_{4+k(n-1)}\\
     %     \overadd{\frac{n-3}{2}}{\tilde\psi}_{5+k} & \ldots & \overadd{\frac{n-3}{2}}{\tilde\psi}_{4+k(n-1)}\\
     %     \overadd{1}{\tilde\psi}_{5+k} & \ldots & \overadd{1}{\tilde\psi}_{4+k(n-1)}\\
     %     \vdots & \ddots & \vdots \\
     %    \overadd{\frac{n-5}{2}}{\tilde\psi}_{5+k} & \ldots &\overadd{\frac{n-5}{2}}{\tilde\psi}_{4+k(n-1)} \\
     %    \overadd{1}{\chi}_{5+k} & \ldots &\overadd{1}{\chi}_{4+k(n-1)} \\
     %     \vdots & \ddots & \vdots \\
     %    \overadd{k}{\chi}_{5+k} & \ldots &\overadd{k}{\chi}_{4+k(n-1)} \\
     %    \overadd{\frac{n-1}{2}}{\tilde\psi}_{5+k} & \ldots & \overadd{\frac{n-1}{2}}{\tilde\psi}_{4+k(n-1)} \\
     %    \vdots & \ddots & \vdots \\
     %    \overadd{k}{\tilde\psi}_{5+k} & \ldots & \overadd{k}{\tilde\psi}_{4+k(n-1)}
     % \end{pmatrix}
     % \circ \zdivtwo \circ C
     % \,,\quad
     \rho_k :=
     \begin{pmatrix}
         \TTtpvec{5+k}\\
         \TTtpvec{6+k} \\
         \vdots \\
         \TTtpvec{4+k(n-1)}
     \end{pmatrix}\,.
 \end{align}
 %
 For this we note that the $ \overadd{p}{r}_A$'s are in $\CKVp$ because each summand in the right-hand side of \eqref{9IX23.w1} is the divergence of a trace-free symmetric tensor, hence is in $\CKVp$.  The vector fields $ \TTtpvec{i}_A$  and
  $ \overadd{i}{s}_{A}$ are in $\CKVp$ by definition. Similarly only the $\CKVp$-part of the vectors $\partial_u^i \xi_A$ enters into $\upsilon_k$ by definition.

  To continue, we need to show that fields $\upsilon_k^{[S]}$ and $\rho_k^{[S]}$ only produce $u_k^{[S]}$; similarly for $\upsilon_k^{[V]}$, $\rho_k^{[V]}$, and $u_k^{[V]}$.
  For this  it can be verified, using the results in Appendices \ref{ss18VIII23.1}-\ref{ss4IX23.2}, that the  operators appearing in $\Lambda_k$ are either products of elliptic, self-adjoint, pairwise commuting operators of the form
 %
 \begin{align}
     % (\zdivtwo \circ C + c)
     % \quad \text{and/ or} \quad
   &  \tilde{L}_{a,c,b} : X \rightarrow X \,, \quad X\in\{S,V\}\,,
   \nonumber
     \\
   &  \tilde{L}_{a,c,b} (\xi) = a \zdivtwo \circ C(\xi) + (\delta_{1b} \TSzlap  + c )\xi
     \,,
     \quad a,c\in \R\,, b\in\{0,1\} \,,
     \label{26IX23.1}
 \end{align}
 %
 where $\delta_{ij}$ is the usual Dirac-delta symbol, or sums thereof.  The decomposition \eqref{4IX23.1} follows.
 % In addition, whenever the operator $\tilde{L}_{a,c}$ appears in $\Lambda_k^{\red{[X]}}$, the factor `$a$' is such that $\tilde{L}_{a,c}$ is elliptic (as an operator acting on $X\in\{S,V\}$).
 }




It follows from \eqref{26IX23.1} that  there exists a complete set of smooth,
 pairwise $L^2$-orthogonal, joint eigenvectors $\eta^{\red{[X]}}_\ell$ of all the $ \tilde{L}_{a,c,b}$'s appearing in $\Lambda^{\red{[X]}}_k$, with a corresponding discrete set of eigenvalues $\lambda^{\red{[X]}}_{a,c,b,\ell}\to_{\ell \to \infty} \infty$. We can therefore write, for $X\in\{S,V\}$,
 %
 \begin{align}
     u^{\red{[X]}}_k = \sum_\ell u^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell \,,\quad
     \upsilon^{\red{[X]}}_k =  \sum_\ell \upsilon^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell
     \,,\quad
     \rho^{\red{[X]}}_k =  \sum_\ell \rho^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell
      \,,
     \label{4IX23.7}
 \end{align}
 %
 and we will show that equation \eqref{4IX23.1} can be solved mode-by-mode:
 %
 \begin{align}
    u_{k,\ell}^{\red{[X]}} = \Lambda^{\red{[X]}}_k \upsilon_{k,\ell}^{\red{[X]}} + \mathcal{N}^{\red{[X]}}_k  \rho_{k,\ell}^{\red{[X]}}
    \iff
     u_{k,\ell}^{\red{[X]}} = \Lambda^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}} \upsilon_{k,\ell}^{\red{[X]}} + \mathcal{N}^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}  \rho_{k,\ell}^{\red{[X]}}    \,.
     \label{26IX23.2}
 \end{align}
 %

 The remaining argument for the solvability of equation \eqref{4IX23.1} is similar to the convenient case.
 We show in Appendix~\ref{ss24IX23.2}
 that the operators $\Lambda_k^{\red{[X]}}$ in \eqref{4IX23.1} are elliptic in the sense of Agmon, Douglis and Nirenberg.
 %
%  $\det \Lambda^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}$ is a polynomial in $\lambda^{\red{[X]}}_{a,c,b,\ell}$.
We also show there that in each line of the matrix $\Lambda^{\red{[X]}}_k$,
the operators lying to the right of the diagonal are of lower order
 than those lying on or to the left of the diagonal. It follows
 \ptcr{not clear if the justification is correct; perhaps should be: it follows from the ADN estimates that ....}
 that $\det \Lambda^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}$ is non-zero for $\ell$ large enough, and therefore there exists $N(k)$ such that we can find a unique solution of \eqref{26IX23.2} with  $\rho^{\red{[X]}}_{k,\ell}=0$ for all $\ell > N(k)$. It remains to show that  \eqref{26IX23.2} can be solved in the finite dimensional space of $u^{\red{[X]}}_k$'s, $\upsilon^{\red{[X]}}_k$'s and $\rho^{\red{[X]}}_k$'s of the form
 %
 \begin{equation}
 \label{26IX23.11}
   u^{\red{[X]}}_k= \sum_{\ell\le N(k) } u^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell
   \,, \quad
   \upsilon^{\red{[X]}}_k= \sum_{\ell\le N(k) }  \upsilon^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell
   \,, \quad
  \rho^{\red{[X]}}_k = \sum_{\ell\le N(k) }  \rho^{\red{[X]}}_{k,\ell} \eta^{\red{[X]}}_\ell
   \,.
 \end{equation}
 %
This is equivalent to the requirement that all the linear maps  obtained by juxtaposing $\Lambda^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}$ and $ \mathcal{N}^{\red{[X]}}_k|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}$ with $\ell < N(k)$ are surjective. This, in turn, is equivalent to the fact that the adjoints of these linear maps have no kernel. In what follows, we leave out the ``$|_{\tilde L_{a,c,b} \mapsto \lambda^{\red{[X]}}_{a,c,b,\ell}}$'' to ease notation.

It turns out that the question of surjectivity is easier to analyse if we carry out a permutation of the rows and columns of the system \eqref{4IX23.1} as follows: let $\sigma_1$ and $\sigma_2$ be permutations of $\{1,2,...,2k\}$ such that the permuted vectors $(\hat{u}_k)_i := (u_k)_{\sigma_1(i)}$ and $(\hat{\upsilon}_k)_i := (\upsilon_k)_{\sigma_2(i)}$ reads
%
\begin{align}
    \hat{u}_k &= (
                \overadd{1}{r}\,,
                \overadd{1}{s} \,,
                \overadd{2}{r} \,,
                \overadd{2}{s} \,,
               \dots \,,
               \overadd{k}{r} \,,
               \overadd{k}{s}
           )^T \,.
           \\
     \hat{\upsilon}_{k} &:=
\left\{
  \begin{array}{ll}
        (
     \upsilon_{k,2} \,,
 \TTtpvec{\frac{9-n}{2}} \,,
 \dots \,,
 \TTtpvec{1}  \,,
 \TTtpvec{4}  \,,
 \dots \,
 \TTtpvec{4+k}
 )^{T [\CKVp]}, & \hbox{$k= \frac{n-3}{2}$;} \\
        (
      \kxi{2}_A \,,
     \upsilon_{k,2} \,,
 \partial^{k_n}_u \kxi{2}_A \,,
 \partial^{k_n-1}_u \kxi{2}_A \,,
 \dots \,,
 \partial_u \kxi{2}_A
     \,,
 \TTtpvec{\frac{9-n}{2}} \,,
 \dots \,,
 \TTtpvec{1}  \,,
 \TTtpvec{4}  \,,
 \dots \,
 \TTtpvec{4+k}
 )^{T [\CKVp]}, & \hbox{$k> \frac{n-3}{2}$.}
  \end{array}
\right.
\end{align}
%%
%{\redc \ptc{old}
%%
%\begin{align}
%    \hat{u}_k &= (
%                \overadd{1}{r}\,,
%                \overadd{1}{s} \,,
%                \overadd{2}{r} \,,
%                \overadd{2}{s} \,,
%               \dots \,,
%               \overadd{k}{r} \,,
%               \overadd{k}{s}
%           )^T \,.
%           \\
%     \hat{\upsilon}_{k} &:=
%     (
%      \kxi{2}_A \,,
%     \upsilon_{k,2} \,,
% \partial^{k_n}_u \kxi{2}_A \,,
% \partial^{k_n-1}_u \kxi{2}_A \,,
% \dots \,,
% \partial_u \kxi{2}_A
%     \,,
% \TTtpvec{\frac{9-n}{2}} \,,
% \dots \,,
% \TTtpvec{1}  \,,
% \TTtpvec{4}  \,,
% \dots \,
% \TTtpvec{4+k}
% )^{T [\CKVp]}
%\end{align}
%%
%}
Then $(\Lambda^{\red{[X]}}_k \, \mathcal{N}^{\red{[X]}}_k)$ is surjective iff
$( \hat{\Lambda}^{\red{[X]}}_k \, \hat{\mathcal{N}}^{\red{[X]}}_k)$
is, where $(\hat{\Lambda}_k^{\red{[X]}})_{ij}:= (\hat{\Lambda}_k^{\red{[X]}})_{\sigma_1(i)\sigma_2(j)}$
and
$(\hat{\mathcal{N}}^{\red{[X]}}_k)_{ij}:= (\hat{\mathcal{N}}^{\red{[X]}}_k)_{\sigma(i)j}$.
The benefit in doing so is that the permuted matrix $( \hat{\Lambda}^{\red{[X]}}_k \, \hat{\mathcal{N}}^{\red{[X]}}_k)^\dagger$ then has a similar structure to that in \eqref{27VII23.w1}. Specifically, it can be verified that $( \hat{\Lambda}^{\red{[X]}}_k \, \hat{\mathcal{N}}^{\red{[X]}}_k)^\dagger = \begin{pmatrix}
     F^{\red{[X]}} \\ G^{\red{[X]}}
\end{pmatrix}$, where $G^{\red{[X]}}$ is given by,
 %
 \begin{align}
     \label{5IX23.w1}
     \left(\begin{array}{l}
            \begin{array}{|cccccc|}
            \hline
               \overadd{1}{\psi}_{\frac{9-n}{2}}            &  \overadd{1}{\chi}_{\frac{9-n}{2}}  & \dots \quad \dots    & \ldots \quad \dots  & \dots\quad\dots\quad \dots\quad\dots   \quad \ldots    &  \, \overadd{k}{\chi}_{\frac{9-n}{2}} \phantom{LL}
               \\
               \vdots           &  \vdots  &     &   &     &  \, \vdots
               \\
               \fbox{ $\overadd{1}{\psi}_{\frac{7-n}{2}+(n-1)}$ } &  \overadd{1}{\chi}_{\frac{7-n}{2}+(n-1)}  & \dots \quad \dots    & \ldots \quad \dots  & \dots\quad\dots\quad \dots\quad\dots      \quad \ldots & \, \overadd{k}{\chi}_{{\frac{7-n}{2}+(n-1)}}
               \\
            \hline
            \end{array}
                \\ \vspace{-.4cm}
        \\
            \begin{array}{|cccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0       &   \hspace{1.5cm}  \overadd{1}{\chi}_{{\frac{9-n}{2}+(n-1)}}    &  \dots   \quad   &  \dots  \quad     & \ldots\quad\dots\quad\dots\quad \ldots \quad\dots\quad \ldots & \overadd{k}{\chi}_{{\frac{9-n}{2}+(n-1)}}
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots        &     \hspace{2cm}\vdots     &        &                                      &                             & \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &   \hspace{1.5cm} \fbox{$\overadd{1}{\chi}_{(n-1)+4} $}     &    \dots \quad   &   \dots  \quad & \ldots\quad\dots\quad\dots\quad \ldots\quad\dots\quad \ldots  & \overadd{k}{\chi}_{(n-1)+4}
              \\
            \hline
            \end{array}
        \\
            \begin{array}{cccccc}
                 & \phantom{\overadd{k}{\chi}_{,k}\qquad\qquad}    &  \phantom{\overadd{k}{\chi}_{}\qquad\qquad\qquad}    & \quad \vdots &   &
            \end{array}
        \\
            \begin{array}{|ccccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &   \hspace{2cm}     & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0        &\hspace{0.3cm}  \overadd{k}{\psi}_{(k-1)(n-1)+5} \quad  & \overadd{k}{\chi}_{(k-1)(n-1)+5}
              \\
             \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots      &       & \vdots        & \ddots \quad\ddots \quad\ddots \quad \ddots \quad \ddots & \vdots        &\, \vdots \quad  & \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &       & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0 &\hspace{0.3cm} \fbox{$\overadd{k}{\psi}_{\frac{7-n}{2}+k(n-1)} $}\quad  & \overadd{k}{\chi}_{\frac{7-n}{2}+k(n-1)}
              \\
            \hline
            \end{array}
        \\ \vspace{-.4cm}
        \\
            \begin{array}{|ccccccc|}
            \hline
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &   \hspace{2cm}     & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0        &\hspace{1.4cm}  0 \quad  & \hspace{1.2cm} \overadd{k}{\chi}_{\frac{9-n}{2}+k(n-1)}
              \\
             \phantom{\overadd{k}{\chi}_{,kkk}} \, \vdots      &       & \vdots        & \ddots \quad\ddots \quad\ddots \quad \ddots \quad \ddots & \vdots        &\hspace{1.4cm} \vdots \quad  & \hspace{1.2cm} \vdots
              \\
              \phantom{\overadd{k}{\chi}_{,kkk}} \, 0      &       & 0        & \ldots \quad\ldots \quad\ldots \quad \dots \quad \dots & 0 &\hspace{1.5cm}  0 \quad  & \hspace{1.2cm} \fbox{$\overadd{k}{\chi}_{k(n-1)+4}$}
              \\
            \hline
            \end{array}
            \end{array}
     \right)\,,
 \end{align}
 %
 where all the operators appearing are understood to be the associated restrictions onto the space $X\in\{S,V\}$.
 In addition, the boxed entries in \eqref{5IX23.w1} are all non-vanishing scalars (cf.\  items (iii) of Sections \peqref{ss26XI22.3} and \peqref{e3IX23.2}). It follows readily that $G^{\red{[X]}}$, and hence
$( \hat{\Lambda}^{\red{[X]}}_k \, \hat{\mathcal{N}}^{\red{[X]}}_k)^\dagger$, has trivial kernel.

\wcb{to do: $\TTt$ part $\alpha \neq 0$}


\newpage




==> RefereeResponse.tex <==
Dear editor, 

We are grateful to the referee for the helpful comments and questions. Here are our responses to the points raised:

1. we have removed the phrase as the referee suggested.

2. when m = 0, there are both gauge-invariant and gauge-dependent charges. The "obstructions" we had in mind in this sentence refers only to those gauge-invariant charges, which becomes gauge-dependent when m is non-vanishing. We have modified the paragraph around this sentence to hopefully better reflect this. 

3. in footnote 1., we stated that the some of the fields in (3.10) are "not independent", because they are related by the Einstein constraint equations. We wrote that this is "irrelevant for our purposes" because in the gluing problem, we assume that the datum given arise from spacetimes satisfying the Einstein equations. In particular, the datum do satisfy the constraint equations, or in the words of the referee, they are compatible.

4. we have removed the problematic expression

In addition to the above changes, we wish to point out that we have modified sections 4.3.1-4.3.2, and added a new section 5, to address the regularity of the fields.

==> WanMacros.tex <==
\usepackage{eufrak}

\newcommand{\mcE}{\red{\mycal{E}}}
\newcommand{\mcN}{\red{\mycal{N}}}

\newcommand{\hyp}{\red{\mycal S}}


\newcommand{\mcD}{\red{\mycal D}}
\newcommand{\mcM}{\red{\mycal M}}
\newcommand{\nmnM}{\red{{}^{n-1}M}}

\newcommand{\red}[1]{{\color{red}#1}}

\DeclareFontFamily{OT1}{rsfs}{}
\DeclareFontShape{OT1}{rsfs}{CGNPm}{n}{ <-7> rsfs5 <7-10> rsfs7 <10-> rsfs10}{}
\DeclareMathAlphabet{\mycal}{OT1}{rsfs}{CGNPm}{n}

\newcommand{\mcU}{\red{\mycal U}}
\newcommand{\mcV}{\red{\mycal V}}
\newcommand{\mcO}{\red{\mycal O}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{figure}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{table}{section}
\renewcommand{\thetable}{\thesection.\arabic{table}}



\newcounter{mnotecount}[section]

\renewcommand{\themnotecount}{\thesection.\arabic{mnotecount}}

%
%\newcommand{\mnotet}[1]%{}
%{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
%$%\!\!\!\!\!\!\,
%\bullet$\themnotecount}}$ \protect\todo[]{$\!\!\!\!\!\!\,\bullet$\protect\themnotecount: #1} }

\newcommand{\mnote}[1]%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize
$%\!\!\!\!\!\!\,
\bullet$\themnotecount}}$ \marginpar{%\color{red}%
\raggedright\tiny\em
$\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }



\newcommand{\ptcr}[1]{{\color{red}\mnote{{\color{red}{\bf ptc:}
#1} }}}
\newcommand{\ptcrt}[1]{{\color{red}\mnotet{{\color{red}{\bf ptc:}
#1} }}}
\newcommand{\ptct}[1]{{\mnotet{{\bf ptc:}
#1} }}

\newcommand{\ptcb}[1]{{\color{blue}\mnote{{\color{blue}{\bf ptc:}
#1} }}}
\newcommand{\ptc}[1]{{\color{magenta}\mnote{{\color{blue}{\bf ptc:}
#1} }}}

\newcommand{\redc}{\color{red} }
\newcommand{\bluec}{\color{blue} }
\newcommand{\blueca}[1]{\color{blue} \ptc{changed or added on #1} }
\newcommand{\ptchange}[1]{\color{blue} \ptc{changed on #1} }
\newcommand{\redca}[1]{\color{red}\mnote{ptc: added or changed on #1} }
\newcommand{\green}[1]{\textcolor{darkgreen}{#1}}

\newcommand{\ptcheck}[1]{ \ptc{checked on #1} }



==> alternativeInduction.tex <==
\ptcr{file alternativeInduction.tex; index shifted compared to the previous one, but the good source term still same notation}
For the sake of induction, let us assume that the fields
$\kphi{\ell}_{AB}$ for $\ell\leq 2p$ are known
 \ptcr{is this the right starting point?}
  and collect them, together with $-\partial_u^p\zhTB_{uA}|_{\tilde\secN_2}$, into a new term $\overset{({p})}{\hat{\tilde X}}_A$, allowing us to rewrite
  the $L^2$-projection  on   $\CKVp$ of
  \eqref{6X22.w8b}  as 
%
\begin{align} 
    \big(\overset{({p-1},0)}{\ochi}_{2p+1} (r_2) +
      \overset{({p-1},1)}{\ochi}_{2p+1} (r_2) P
    \big)
     \kphi{2p+1}{}^{[\TTt^\perp]}_{AB}
 &
  +
   \overset{({p-1},0)}{\ochi}_{2p+2} (r_2) 
    \kphi{2p+2}{}^{[\TTt^\perp]}_{AB}
    \nonumber
\\
    &\quad
    =
    (\zdivtwo)^{-1} 
    \big(
 \partial_u^{p}\kxi{2}{} 
    -
 \overset{({p-1})}{\hat{\tilde X}} {}
 \big)_{AB}^{[\CKVp]}
    \,.
    \label{12VII23.7}
\end{align} 
%


We similarly have 
 \ptcr{needs reorganising, this appears only in the next section}
\ptcheck{20XI, magical}
%
\begin{align}  
     \Big(
      \overset{({p},0)}{\opsi}_{2p+1} 
      & (r_2) 
       + \overset{({p},1)}{\opsi}_{2p+1} (r_2) P + \overset{({p},2)}{\opsi}_{2p+1} (r_2) P^2 \
       \Big)
        \kphi{2p+1}{}^{[\TTt^\perp]}_{AB} 
      \nonumber
\\ 
  &
   +
 (\overset{({p},0)}{\opsi}_{2p+2} (r_2) 
  + \overset{({p},1)}{\opsi}_{2p+2} (r_2) P )\kphi{2p+2}{}^{[\TTt^\perp]}_{AB}
     \nonumber
\\
   &=
  \partial^p_u \hBo_{AB}^{[\TTt^\perp]}|_{\tilde{\secN}_2}  
  - 
    \overadd{p}{\tilde\Psi}{}^{[\TTt^\perp]}_{AB}(r_2, x^A)
    - 2 r_2^2  \TS [\zspaceD_{\tdA}\partial_{\tdu}^{p}\kxi{2}_B^{[\CKVp]}]
    %+ r_2 \zspaceD^A \TS [\zspaceD_{\tdA}\zspaceD_{\tdB}\zspaceD_{\tdC}\partial_{\tdu}^{p-1}\kxi{2}^C]
\,,
       \label{12VII23.6}
\end{align}
%
This gives a system of equations for $(\kphi{2p+1}{}^{[\TTt^\perp]},\kphi{2p+2}{}^{[\TTt^\perp]})$, with principal part
%
\begin{equation}\label{12VII23.11}
  \left(
              \begin{array}{cc}
      \overset{({p-1},1)}{\ochi}_{2p+1} (r_2) P & 
   \overset{({p-1},0)}{\ochi}_{2p+2} (r_2) 
     \\
                \overset{({p},2)}{\opsi}_{2p+1} (r_2) P^2
                 & 
 \overset{({p},1)}{\opsi}_{2p+2} (r_2) P \\
              \end{array}
            \right)\,.
\end{equation}
%
Let us check  ellipticity in the sense of Agmon-Douglis-Nirenberg. For this we set 
%
\begin{equation}\label{12VII23.13}
  s_1=0\,,\
    s_2 =2
  \,,\ 
  r_1=2 \,,\
  r_2 = 0
  \,,
\end{equation}
%
so that the $(i,j)$'th entry of the matrix \eqref{12VII23.11} is an operator of order $s_i+r_j$. The system is thus elliptic   if the matrix 
%
\begin{equation}\label{12VII23.11}
 A:=
   \left(
              \begin{array}{cc}
      \overset{({p-1},1)}{\ochi}_{2p+1} (r_2)  & 
   \overset{({p-1},0)}{\ochi}_{2p+2} (r_2) 
     \\
                \overset{({p},2)}{\opsi}_{2p+1} (r_2)  
                 & 
 \overset{({p},1)}{\opsi}_{2p+2} (r_2)  \\
              \end{array}
            \right)
            %\,.
\end{equation}
%
is invertible (cf., e.g., \cite{Carson}.) However, the determinant of $A$ is zero by \eqref{8XI22.w4b}, thus ellipticity does not hold.
 \ptcr{give ref to original work or morrey, see also refs in the paper with Marc on analyticity}


==> decomp.tex <==
Let $\xi_A\in \CKVp$, and consider its scalar-vector decomposition:
%
\begin{equation}\label{4X23.1}
  \Box_{\hring} \phi = \zspaceD_A \xi^A
  \,,
  \quad
  \xi^{[S]}_A  = \zspaceD_A \phi
  \,,
  \quad
  \xi^{[V]}_A  = \xi_A - \zspaceD_A \phi 
  \,.
\end{equation}
%
Then $\xi^{[S]}_A $ will   be in $\CKVp$ if and only if for all conformal Killing $\chi^A$ vectors we have
%
\begin{equation}\label{4X23.2}
  0 =  \int_{\secN} \chi^A \zspaceD_A \phi 
    \,\sm =  - \int_{\secN}  \phi \zspaceD_A\chi^A 
    \,\sm 
    \,.
\end{equation}
%
This will certainly be the case if either a) $\CKV=\{0\}$ (which is the case on negatively Ricci-curved manifolds), or b) $\CKV =\KV$ (which is the case on  Ricci-flat manifolds). 
 \ptcr{certainly on tori, but for all Ricci flat? to check} 

On $S^n$ the functions $\zspaceD_A\chi^A $ are linear combinations of $\ell=1$ spherical harmonics, and so \eqref{4X23.1} will fail unless the projection of $\zspaceD_A \xi^A$ on the space spanned by $\ell=1$ harmonics vanishes:
%
\begin{equation}\label{4X23.3}
  (\zspaceD^A \xi_A )^{[=1]} = 0
  \,.
\end{equation} 
%
Now, still on $\S^n$, the proper conformal Killing vectors are gradients of $\ell=1$ spherical harmonics. So let $\chi_A = \zspaceD_A \varphi \in \CKV$, since  $\xi_A\in \CKVp$ by hypothesis we have for all such $\chi_A$'s
%
\begin{equation}\label{4X23.2}
  0 =  \int_{\secN} \xi^A \zspaceD_A \varphi
    \,\sm =  - \int_{\secN}  \varphi \zspaceD_A\xi^A
    \,\sm
    \,,
\end{equation}
%
which implies that \eqref{4X23.3} holds.

Since $\CKVp$ is a vector space, if  $\xi_A$ is in $\CKVp$ and \eqref{4X23.2} holds, then the right-hand side of that  equation in \eqref{4X23.1} which defines $\xi^{[V]}_A$ will be in $\CKVp$, and so will be $\xi^{[V]}_A$. 


==> du2hABcharge.tex <==
%
\wcb{Not sure; below to be rewritten or discarded \\ -- \\ ptc: let's leave it in for the moment, I have to think this through, is relevant for the torus or in higher dims}
Let $\vp{T}_{AB}$ denote the vector part and $\TT{T}_{AB}$ denote the transverse traceless part of any symmetric, traceless tensor $T_{AB}$. In the case when $\secN$ is not $S^2$, \eqref{26VII22.2} determines $\ip{\hkappaone}{\TT{\wh}_{AB}}$ in terms of $\partial_u\TT{\hBo}_{AB}|_{\tilde\secN_2}$. Hence there are no free fields in the $TT$ part of \eqref{26VII22.4}; it is a constraint equation for $\partial_u^2\TT{\hBo}_{AB}|_{\tilde\secN_2}$.
Alternatively, we can also see that $\partial_u^2\TT{\hBo}_{AB}|_{\tilde\secN_2}$ is fully constrained from \eqref{eq:31III22.3p0}, reproduced here:
%
\begin{align}
   &  \partial_r \Big[r \partial_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \zhTB_{AB}
     -  \frac{1}{2 r}  V   \zhTB_{AB}
     -\frac{1}{2r^{2}}\partial_r\big(r^2 \TS [\zspaceD_A\hBo_{uB}]\big)
     \Big]
      \nonumber
\\
     	&\quad
      =
       -\frac{1}{2}  \partial_r  (  V/r)  \zhTB_{AB}
        -\frac{1}{2}\partial_r\big(r^{-2}P\hBo_{AB}\big)
        \,.
        \phantom{xxx}
\end{align}
%
The $TT$ part of the above reads,
%
\begin{align}
\label{23VIII22.w1}
    \partial_r \TT{\Big[r \partial_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \zhTB_{AB}
     -  \frac{1}{2 r}  V   \zhTB_{AB}
     \Big]}
      =
       -\frac{1}{2}  \partial_r  (  V/r)  \TT{\zhTB}_{AB}
        \,.
        \phantom{xxx}
\end{align}
%
Taking the $u$-derivative of \eqref{23VIII22.w1} gives,
%
\begin{align}
    & \partial_r \TT{\Big[r \partial^2_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \partial_u\zhTB_{AB}
     -  \frac{1}{2 r}  V   \partial_u\zhTB_{AB}
     \Big]}
     \nonumber
\\
    &\qquad
      =
       -\frac{1}{2}  \partial_r  (  V/r)  \partial_u\TT{\zhTB}_{AB}
       + \red{\alpha^2} r\partial_r \TT{\Big[r \partial_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \zhTB_{AB}
     -  \frac{1}{2 r}  V   \zhTB_{AB}\big)
     \Big]}
     + \red{\alpha^2} r \frac{1}{2}  \partial_r  (  V/r)  \TT{\zhTB}_{AB}
        \nonumber
\\
   &\qquad
      =\partial_r(\red{\alpha^2} \partial_u \TT{\hBo}_{AB})
      - \red{\alpha^2} r\partial_r \TT{\Big[
      \frac{ 1}{2}  V  \partial_r \zhTB_{AB}
     +  \frac{1}{2 r}  V   \zhTB_{AB}\big)
     \Big]}
     + \red{\alpha^2} r \frac{1}{2}  \partial_r  (  V/r)  \TT{\zhTB}_{AB}
     \,,
\end{align}
%
which can be integrated to give,
%
\begin{align}
    &\TT{\Big[\big(r \partial^2_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \partial_u\zhTB_{AB}
     -  \frac{1}{2 r}  V   \partial_u\zhTB_{AB}
     -\red{\alpha^2} \partial_u \hBo_{AB}\big)}
     \Big]_{r_1}^r
     \nonumber
\\
    &\quad
    = \int \TT{\bigg(
   \frac{1}{2} \red{\alpha^2} \left(\red{\alpha^2} s^2-\twoscsign \right)\partial_s^2\hBo_{AB}(s)
   +\frac{\red{\alpha^2} \twoscsign }{s} \partial_s \hBo_{AB}(s)
   -\left(\alpha^4+\frac{\red{\alpha^2} \twoscsign }{s^2}\right) \hBo_{AB}(s)
    \bigg)}
    ds
         \nonumber
\\
    &\quad
    =\bigg[\frac{1}{2} \red{\alpha^2} \left(\red{\alpha^2} s^2-\twoscsign \right)\partial_s\TT{\hBo}_{AB}(s)\bigg]_{r_1}^r
    + \int \TT{\bigg( \red{\alpha^2}(\frac{\twoscsign}{s}-\red{\alpha^2} s) \partial_s \hBo_{AB}(s)
   -\left(\alpha^4+\frac{\red{\alpha^2} \twoscsign }{s^2}\right) \hBo_{AB}(s)
    \bigg)}
    ds
     \nonumber
\\
    &\quad
    =\bigg[\frac{1}{2} \red{\alpha^2} \left(\red{\alpha^2} s^2-\twoscsign \right)\partial_s\TT{\hBo}_{AB}(s)+\red{\alpha^2}(\frac{\twoscsign}{s}-\red{\alpha^2} s)\TT{\hBo}_{AB}(s)\bigg]_{r_1}^r\,.
\end{align}
%
This is a constraint equation for $\partial_u^2\TT{\hBo}_{AB}|_{\secN_2}$ in terms of Bondi data of lower order. 

==> end2.tex <==
%\backmatter
%\bibliographystyle{/usr/local/lib/texmf/bibtex/bst/amsplain}
%\bibliography{$HOME/prace/references/hip_bib,%
%$HOME/prace/references/reffile,%
%$HOME/prace/references/vienna,%
%$HOME/prace/references/newbiblio,%
%$HOME/prace/references/newbiblio2,%
%$HOME/prace/references/netbiblio,%
%$HOME/prace/references/bibl,%
%$HOME/prace/references/howard}
%\bibliographystyle{JHEP}
%\bibliographystyle{amsplain}
\bibliography{../../references/hip_bib,%
../../references/reffile,%
../../references/newbiblio4,%
../../references/newbiblio,%
../../references/newbiblio2,%
../../references/besse2,%
../../references/bibl,%
../../references/howard,%
../../references/bartnik,%
../../references/myGR,%
../../references/newbib,%
../../references/Energy,%
../../references/chrusciel,%
../../references/dp-BAMS,%
../../references/prop2,%
../../references/netbiblio,%
../../references/besse}
\end{document}


==> recursionPTC.tex <==
\section{Recursion formulae}
 \label{App14VIII22.2}

Recall that
%
$$
 V = r \twoscsign - {\alpha^2} r^3 \red{-2m}
  \,.
$$
%
We want to show
 \ptc{not sure what the most useful form of the recursion is; \eqref{18VI22.3pc} an unconclusive attempt}
%
\begin{align}
\label{18VI22.3pc}
 \partial_u^i \hBo_{AB}  &=
    \overadd{i}{\Psi}_{AB}(u,r, x^A)
     + \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k }{V}(P)r^{-k} \partial_j\hBo_{AB}	
     +
      \int_{r_1}^{r}
       \sum_{j=0}^i
       \overadd{i,j}{W} (r,P)s^{-j} \hBo_{AB}
        \red{\, ds}
        \,,
        \phantom{xxx}
        \\
  \partial_u^i  \zhTB_{uA}  &=
    \overadd{i}{X}_{A}(u,r, x^A)
     	+ \sum_{0\leq j+k\leq i,k\ne i}
           \overadd{i,j,k}{\chi}(r)\partial_r^j \zspaceD^B P^k \hBo_{AB}
     	+
     \zspaceD^B
      \int_{r_1}^{r}
       \sum_{j=0}^{i }
       \overadd{i,j}{\chi} (s,r)P^j \hBo_{AB}
        \red{\, ds}
        \,,
         \label{18VI22.1pa}
       \phantom{xxx}
\\
\label{18VI22.3p}
 \partial_u^i \hBo_{AB}  &=
    \overadd{i}{\Psi}_{AB}(u,r, x^A)
     + \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k}{\psi}(r)\partial_r^j P^k \hBo_{AB}	
     +
      \int_{r_1}^{r}
       \sum_{j=0}^i
       \overadd{i,j}{\psiP} (s,r) P^j \hBo_{AB}
        \red{\, ds}
        \,,
        \phantom{xxx}
        \\
  \partial_u^i  \zhTB_{uA}  &=
    \overadd{i}{X}_{A}(u,r, x^A)
     	+ \sum_{0\leq j+k\leq i,k\ne i}
           \overadd{i,j,k}{\chi}(r)\partial_r^j \zspaceD^B P^k \hBo_{AB}
     	+
     \zspaceD^B
      \int_{r_1}^{r}
       \sum_{j=0}^{i }
       \overadd{i,j}{\chi} (s,r)P^j \hBo_{AB}
        \red{\, ds}
        \,,
         \label{18VI22.1p}
       \phantom{xxx}
\\
\label{4XI22.w1p}
 \partial_u^i q_{AB} &=
  \red{ \overadd{i}{\Phi}_{AB}(u,r, x^A)
    	+ \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k}{\phi}(r)\partial_r^j
    P^k \hBo_{AB}
    	+
     \int_{r_1}^{r}
      \sum_{j=0}^{i }
      \overadd{i,j}{\phi} (s,r)P^j \hBo_{AB}}
       \red{\, ds}
       \,,
       \phantom{xxx}
\end{align}
%
Let us write $\tkfbd$ for terms known from ``boundary data at $r_1$ ''.  We rewrite \eqref{24VII22.61} as
%
\begin{eqnarray}
\label{eq:31III22.3p}
      \partial_u h_{AB}
      &=&
      \tkfbd
      +
      r \Bigg[
     \frac{1}{2}\Big[
        V  \partial_r \zhTB_{AB}
     +   \frac{1}{r}  V   \zhTB_{AB}
     \Big]
     \nonumber
\\
&&
            + \int_{r_1}^r
     \Big[
      \red{( \frac{\alpha^2}{s} -\frac{m}{s^4} )}\hBo_{AB}
       +
          \bigg(\frac{1}{ 3s r^{2}}
    +\frac{2 r}{3 s^4}\bigg) \TS \big[
          \zspaceD_A   \zspaceD^C \hBo_{BC}
       \big]
       \Big]\Bigg]
        \red{\, ds}
        \nonumber
\\
      &=&
     \frac{r( \twoscsign r- {\alpha^2} r^3 \red{-2m} ) }{2 }\Big[
         \partial_r(r^{-2} h_{AB})
     +   \frac{1}{r^3}    h_{AB}
     \Big]
     \nonumber
\\
&&
            +  \int_{r_1}^r
     \Big[
       \underbrace{(\frac{{\alpha^2}r }{s} -\red{\frac{m r}{s^4})}}_{\overadd{1}{\psi}} \hBo_{AB}
       +
          \underbrace{
           \bigg(\frac{1}{ 3s r }
    +\frac{2 r^2 }{3 s^4}\bigg)
    }_{\overadd{1,1}{\psi}(s,r)} P h  _{AB}
       \big]
       \Big]
        ds
        + \tk
        \,.
\label{14VIII22.1}
\end{eqnarray}
%
We also have
%
\begin{align}
    r^4\partial_r\zhTB_{uA}|_r = r_1^4 \partial_r\zhTB_{uA}|_{r_1}+\big[\zspaceD^B\hBo_{AB}\big]_{r_1}^{r} - 2\int_{r_1}^r \hat{\kappa}_1(s) \zspaceD^B\hBo_{AB}\,ds
    \label{25VII22.3p}
\end{align}
%
%
\begin{align}
   &  \partial_r \Big[\underbrace{r \partial_u \zhTB_{AB}
     - \frac{ 1}{2}  V  \partial_r \zhTB_{AB}
     -  \frac{1}{2 r}  V   \zhTB_{AB}
     -\frac{1}{2r^{2}}\partial_r\big(r^2 \TS [\zspaceD_A\hBo_{uB}]\big)
     +\frac{1}{2}P\zhTB_{AB}}_{\blue{:=q_{AB}}}\Big]
      \nonumber
\\
     	&\quad
      =
        \big(
        \frac{ {\alpha^2}}{r} - \frac{m}{r^4}
       \big)
        \hBo_{AB}
        \,.
        \phantom{xxx}
        \label{3IX22.1p}
\end{align}
%
It is convenient to separate the terms involving $\alpha$ and $\red{m}$ from the remaining ones:
%
\begin{eqnarray}
\label{eq:31III22.3p}
      \partial_u h_{AB }
      &=&
     \frac{\twoscsign }{2 }\Big[
        \partial_r h_{AB}
     - \frac{1}{r }    h_{AB}
     \Big]   +  \int_{r_1}^r
           \bigg(\frac{1}{ 3s r }
    +\frac{2 r^2 }{3 s^4}\bigg)
     P h  _{AB}
        \red{\, ds}
        \nonumber
\\
 &&
     - (\frac{  {\alpha^2} r^2 }{2 }+\red{\frac{2m}r} )\Big[
        \partial_r h_{AB}
     - \frac{1}{r }    h_{AB}
     \Big]   +  \int_{r_1}^r
        (\frac{{\alpha^2}r }{s}  \red{-\frac{mr}{s^4})} \hBo_{AB}
        \red{\, ds}
        + \tk
        \,.
\label{14VIII22.3}
\end{eqnarray}
%
 \ptcheck{14VIII22 }
Set  $\overadd{1,0}{\psi}:= \overadd{1}{\psi}$.
When $\alpha = 0$, inserting \eqref{14VIII22.3}
 into the $u$-derivative of \eqref{18VI22.3} leads to
%
\begin{eqnarray}
 \partial_u^{i+1} \hBo_{AB}
  &=&
 \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k}{\psi}(r)\partial_r^j P^k \partial_u\hBo_{AB}
 %    \nonumber
%     \\
%     &&	
+
       \sum_{j=0}^i \int_{r_1}^{r}
       \overadd{i,j}{\psiP} (s,r)P^j \partial_u\hBo_{AB}
        \red{\, ds}
        +  \tkfbd
         \nonumber
\\
  &=&
 \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k}{\psi}(r)\partial_r^j P^k
\Big[
  \frac{\twoscsign }{2 }\Big[
        \partial_r h_{AB}
     - \frac{1}{r }    h_{AB}
     \Big]   +  \int_{r_1}^r
           \bigg(\frac{1}{ 3s r }
    +\frac{2 r^2 }{3 s^4}\bigg)
     P h  _{AB}
        \red{\, ds}\Big]
        \nonumber
\\
    &&	
 +
       \sum_{j=0}^i \int_{r_1}^{r}
      \underbrace{
        \overadd{i,j}{\psiP} (s,r)P^j
       \Bigg[
  \frac{\twoscsign }{2 }\Big [
        \partial_s h_{AB}
        }_{\mbox{integrate by parts}}
     - \frac{1}{s }    h_{AB}
     \Big]_s   +  \int_{r_1}^s
           \bigg(\frac{1}{ 3y s }
    +\frac{2 s^2 }{3 y^4}\bigg)
     P h  _{AB}|_y
        dy
        \Bigg]
        ds
        \nonumber
\\
 &&
        +  \tkfbd
         \nonumber
\\
  &=&
 \sum_{0\leq j+k\leq i,k\ne i} \overadd{i,j,k}{\psi}(r)\partial_r^j P^k
\Big[
  \frac{\twoscsign }{2 }\Big[
        \partial_r h_{AB}
     - \frac{1}{r }    h_{AB}
     \Big]
        +    \int_{r_1}^r
           \bigg(\frac{1}{ 3s r }+\frac{2 r^2 }{3 s^4}\bigg)
     P h  _{AB}
        \red{\, ds}\Big]
        \nonumber
\\
    &&	
    +
      \frac 12  \sum_{j=0}^i
       \overadd{i,j}{\psiP} (s,r) \big|_{s=r}P^j
        h_{AB}
 +
       \sum_{j=0}^i \int_{r_1}^{r}
      \big(-\frac \twoscsign 2 \partial_s \overadd{i,j}{\psiP} (s,r)
      - \frac {\twoscsign}{2 s}
       \overadd{i,j}{\psiP} (s,r)
       \big)
        P^j   h_{AB}\big|_s
        ds
        \nonumber
\\
        &&
        +
        \underbrace{ \int_{r_1}^{r}
         \overadd{i,j}{\psiP} (s,r)  \int_{r_1}^s
           \bigg(\frac{1}{ 3y s }
    +\frac{2 s^2 }{3 y^4}\bigg)
     P^{j+1} h  _{AB}|_y
        dy
        \, ds
        }_{
    \displaystyle
     \int_{r_1}^{r} \bigg(\int_{s}^r
     \bigg(\frac{1}{ 3y s }
    +\frac{2 y^2 }{3 s^4}\bigg)
     \overadd{i,j}{\psiP} (y,r)
        dy
        \bigg)
     P^{j+1} h  _{AB}|_s
        \red{\, ds}
        }
%        \nonumber
%\\
% &&
        +  \tkfbd
        \,.
\label{14VIII22.6}
\end{eqnarray}
%



%Of key interest are the terms
% \ptcr{consider reducing duplicate information}
%%
%\begin{equation}\label{15VIII22.1}
% a_j s^{-i-3} \ \mbox{ in $\overadd{i,j}{\psiP}$, }
%\end{equation}
%%
% with $i\ge 1$.
%%We find
%\begin{enumerate}
%  \item when $i=1$, the term $ \overadd{1,0,0}{\psi}(r) =
%     - \frac{1}{2r} \left(\red{\twoscsign - {\alpha^2} r}^2\right)$ induces
%      \ptcr{does not agree with \eqref{3VIII22.2}}
%%
%$$
% - \frac{3}{4r} \left(\red{\twoscsign - {\alpha^2} r}^2\right)
% s^{-4}
% \ \mbox{ in $\overadd{2,1 }{\psiP}$;}
%$$
%%
%  \item and for all $i\ge 1$, a
One finds that
%a term \eqref{15VIII22.1} induces a term
%\ptcheck{15VIII22, together}
%%
%$$
% a_j
%   \frac{i+\red{2}}{2}
% s^{-i-4}
% \ \mbox{ in $\overadd{i+1,j }{\psiP}$ and } \
% a_j
% \frac{i+2}{i(i+3)}
% s^{-i-4}
% \ \mbox{ in $\overadd{i+1,j+1}{\psiP}$.}
%$$
%%
%More generally,
a term
%
\begin{equation}\label{16VIII22.w1}
 a_i s^{-\ell} \ \mbox{ in $\overadd{k,i}{\psiP}$ }
\end{equation}
%
 with $\ell\not \in \{0,3\}$  induces  terms $s^{-1}$, $s^{-4}$ and
%
\begin{equation}\label{16VIII22.12}
 a_i \twoscsign
   \frac{\ell-1}{2}
 s^{-(\ell+1)}
 \ \mbox{ in $\overadd{k+1,i }{\psiP}$ and } \
 a_i
 \frac{\ell-1}{\ell(\ell-3)}
 s^{-(\ell+1)}
 \ \mbox{ in $\overadd{k+1,i+1}{\psiP}$.}
\end{equation}
%
Identical formulae apply to the $\overadd{k,i}{\chi}$'s. In particular
 \ptcheck{ 22VIII by wan}
%
\begin{equation}\label{19VIII22.2}
  \overset{(k,k)}{\psiP}(s,r) =
  \underbrace{\frac{2 (k+1)! r^2 }{(k+2)! (k-1)! }
   }_{=:\overset{(k,k)}{\psiP}_{k+3}(r)}
    \frac{1}{ s^{k+3}} + \ldots
   \,,
   \quad
  \overset{(k,k)}{\chi} =
  \underbrace{
   \frac{ (k+2)! }{(k+3)! (k )! }
   }_{=:\overset{(k,k)}{\chi}_{k+4}}
    \frac{1}{ s^{k+4}} + \ldots
   \,.
\end{equation}
%
Moreover since we had (cf.~\eqref{3VIII22.2})\ptcr{To be checked}
%
\begin{equation}
    \overadd{2,0}{\opsi}_{5}(r) = 0 =: 2r^2 \overadd{0,-1}{\ochi}_{5}(r) \,,\quad
    \overadd{2,1}{\opsi}_{5}(r) =2r^2 \overadd{1,0}{\ochi}_{5}(r)
    \,,\qquad
    \overadd{2,2}{\opsi}_{5}(r) = 2r^2\overadd{1,1}{\ochi}_{5}(r)\,,
\end{equation}
%
it follows by induction from \eqref{16VIII22.12} that
\begin{equation}
    \overset{(i,j)}{\opsi}_{i+3}(s,r) = 2 r^2 \, \overset{(i-1,j-1)}{\ochi}_{i+3}(s,r)
    \label{3IX22.w1}
\end{equation}
%
where $\overset{(i,j)}{\opsi}_{i+3}$ and $\overset{(i-1,j-1)}{\ochi}_{i+3}$ are, as defined in \eqref{18VIII22.w1} in the main text, the coefficients of $1/s^{i+3}$ in $\overset{(i,j)}{\psi}$ and $\overset{(i-1,j-1)}{\chi}$ respectively.

In addition since
%
\begin{equation}
    \overadd{1,0}{\chi}(s,r) = \frac{{\alpha^2} \hkappaone(s)}{2 r^2 }+\frac{\twoscsign\hkappafive(s) }{2}\,,
    \quad
    \overadd{1,1}{\chi} (s,r) = \frac{\hkappafive(s)}{4 }-\frac{\hkappaone(s)}{4 r^4 }\,,
\end{equation}
%
(cf.\ \eqref{3VIII22.2}) it follows by induction that
%
\begin{equation}
    \overadd{i,j}{\ochi}_{i+3}(s,r) = 0\,.
    \label{2IX22.w1}
\end{equation}
%


